TeachCLIP: Multi-Grained Teaching for Efficient Text-to-Video Retrieval

For text-to-video retrieval (T2VR), which aims to retrieve unlabeled videos by ad-hoc textual queries, CLIP-based methods are dominating. Compared to CLIP4Clip which is efficient and compact, the state-of-the-art models tend to compute video-text similarity by fine-grained cross-modal feature interaction and matching, putting their scalability for large-scale T2VR into doubt. For efficient T2VR, we propose TeachCLIP with multi-grained teaching to let a CLIP4Clip based student network learn from more advanced yet computationally heavy models such as X-CLIP, TS2-Net and X-Pool . To improve the student's learning capability, we add an Attentional frame-Feature Aggregation (AFA) block, which by design adds no extra storage/computation overhead at the retrieval stage. While attentive weights produced by AFA are commonly used for combining frame-level features, we propose a novel use of the weights to let them imitate frame-text relevance estimated by the teacher network. As such, AFA provides a fine-grained learning (teaching) channel for the student (teacher). Extensive experiments on multiple public datasets justify the viability of the proposed method.

==> backup.tex <==


\textbf{Pearson Distance.} 
 The pearson correlation coefficient is used to calculate the cosine similarity of two centered vectors. We define the $\rho _p(\mathbf{a},\mathbf{b})$ as the pearson correlation coefficient between two N-dimension distributions $\mathbf{a}$ and $\mathbf{b}$, which is more robust to distribution changes. The specific formula is as follows:
 
\begin{equation} \label{eq:peasondefine}
\rho_p(\mathbf{a},\mathbf{b})=\frac{\sum_{i=1}^{N}(\mathbf{a}_i-\bar{\mathbf{a}})(\mathbf{b}_i-\bar{\mathbf{b}})}{\sqrt{\sum_{i=1}^{N} (\mathbf{a}_i-\bar{\mathbf{a}})^2 \sum_{i=1}^{N} (\mathbf{b}_i-\bar{\mathbf{b}})^2}}
\end{equation}

Here $\bar{\mathbf{a}}$ and $\bar{\mathbf{b}}$ represent the mean value of $\mathbf{a}$ and $\mathbf{b}$. The Pearson Distance is defined as $d_p(\mathbf{a},\mathbf{b}) = 1-\rho _p(\mathbf{a},\mathbf{b})$.



We use CLIP4Clip\cite{clip4clip} as a baseline student architecture, due to its low computational and offline storage costs. 
On the visual side, it is composed of an frame encoder and temporal encoder module, and the text side is a text encoder module. 
Although it can exploit the sequential information between frames by the temporal encoder, we argue the current architecture design doesn't consider the importance of different frames.
Therefore, we propose a attentional feature aggregation ($AFA$) module to reasonably assign weights for different frames, which is very lightweight and almost doesn't affect the inference speed.

The detailed structure of the $AFA$ is shown in Fig.\ref{fig:structure}.
Starting with the frame-level features $\mathbf{f}$ extracted by CLIP, $\Phi$ is obtained through the temporal encoder module.
We can obtain weights $\mathbf{w}=\{w_1, \ldots, w_m\}$ of different frames by passing $\Phi$ through $AFA$.
The scale operation controls the steepness of the frame weight distribution, which means it is used to balance the same weight for all frames or very high weight for only one frame.
Finally, we sum $\Phi$ with $\mathbf{w}$ as the weight to get video-level features.

\begin{figure}[ht!]
%   \setlength{\abovecaptionskip}{5pt}
  \centering  \includegraphics[width=\columnwidth]{figures/structure}
  \caption{\textbf{The visual feature re-learning module of our CLIP-based text-to-video retrieval network}. The module consists of 4$\times$ Transformer blocks, which exploits inter-frame information to enhance the original frame-level features $\{f_1, \ldots, f_m\}$, and a simple attentional feature aggregation (AFA) block that weightedly combines the frame-level features. AFA, with its produced weights $\{w_1, \ldots, w_m\}$ supervised by a specific teacher network, provides an effective mean for fine-grained knowledge distillation from the teacher network to our network.}
  \label{fig:structure}
\end{figure}



\subsection{Teacher Models} \label{ssec:teacher}


We use XCLIP\cite{xclip} and TS2Net\cite{ts2net} as teacher models, because these two models achieve significantly better performance than CLIP4Clip by fine-grained video text interaction, which brings the increase of computational complexity and offline storage. So we distill these two teachers to make the student model achieve a trade off between performance and efficiency.


Given a batch of $B$ pairs randomly sampled from the dataset, we use the student model to extract video features and text features respectively. 
We calculate the cosine score of a text and video feature as the cross-modal similarity in Eq.\ref{eq:cosine}, where $M(i,j)$ represents the similarity between the i-th text and the j-th video in the similarity matrix.
\begin{equation} \label{eq:cosine}
M(i,j) = \frac{\mathbf{t}_{i}^{T}\mathbf{v}_{j}}{\left \| \mathbf{t}_{i} \right \|\left \| \mathbf{v}_{j} \right \|}
\end{equation}




\noindent $\bullet$  W2VV++\cite{w2vv++} conducts once 2048-dimension floating point vector multiplication for each video-text pair similarity calculations. \\
\noindent $\bullet$ DualE\cite{dualencoding} conducts a video-text similarity calculation based on 2048-dimension vectors. \\
\noindent $\bullet$ CE\cite{ce} conducts 9 video-text similarity calculations in different common space based on 768-dimension vectors.
\noindent $\bullet$ SEA\cite{sea} conducts 5 video-text similarity calculations in different common space based on 2048-dimension vectors. \\
\noindent $\bullet$ MMT\cite{mmt} conducts 7 video-text similarity calculations in different common space based on 512-dimension vectors. \\
\noindent $\bullet$ TeachText\cite{teachtext} conducts a video-text similarity calculation based on 768-dimension vectors. \\
\noindent $\bullet$ CenterCLIP\cite{centerclip} conducts 3$\sim$15 segment-text similarity calculations for each video-text pair based on 512-dimension vectors. \\
\noindent $\bullet$ CLIP4Clip\cite{clip4clip} conducts a video-text similarity calculation based on 512-dimension vectors. \\
\noindent $\bullet$ TS2-Net\cite{ts2net} conducts 12$\sim$64 frame-text similarity calculations for each video-text pair based on 512-dimension vectors. \\
\noindent $\bullet$ X-CLIP\cite{xclip} conducts 1 video-text, 12$\sim$64 frame-text, 32$\sim$64 video-word and 32x12$\sim$64x64 frame-word  similarity calculations for each video-text pair based on 512-dimension vectors. \\
\noindent $\bullet$ X-Pool\cite{xpool} conducts 12 frame-text similarity calculations based on 512-dimension vectors. Then, 12 similarity scores is adjusted to 12 frame weights by softmax. The fusion feature is obtained by performing 12 times of weight-feature dot product and 11 times of feature vector addition. The fusion feature is multiplied by 512x512 matrix to obtain the final video feature. Finally, the video-text similarity calculation based on 512-dimension vectors.


==> cvpr2023-author_kit-v1_1-1/ablation.tex <==


%\subsection{Ablation Study} \label{ssec:ablation}

Recall that the essence of TeachCLIP is to let a stronger teacher network to teach a computationally efficient student network for better retrieval performance. Hence, TeachCLIP needs to be evaluated along multiple dimensions including the choice of the teacher, the choice of the student, and how the teaching process is executed. 


\textbf{Choice of the teacher network}.  We have X-CLIP\footnote{\url{https://github.com/xuguohai/X-CLIP}} \cite{xclip}, TS2-Net\footnote{\url{https://github.com/yuqi657/ts2_net}} \cite{ts2net} and X-Pool\footnote{\url{https://github.com/layer6ai-labs/xpool}} \cite{xpool} in our shortlist, as they are open-source, provide both video-text and frame-text similarity scores, and report leading performance on multiple datasets. Our experiments show that the performance of TS2-Net is somewhat unstable: better than CLIP4Clip on MSRVTT-1k (SumR 200.5 versus 195.5) and MSRVTT-3k (153.6 versus 150.1), yet worse on MSVD (204.9 versus 206.6) and ActNetCap (190.4 versus 194.1). As for X-Pool, we find that its official code requires computing a big cross-modal similarity matrix between all test videos and texts on a single GPU. Consequently, X-Pool is computationally feasible on MSRVTT-1k only. As such, we choose X-CLIP as the default teacher, unless otherwise stated.

As shown in Table \ref{table:ablation},  the student network \emph{without} teaching (Setup\#2) scores SumR of 196.3. By the proposed multi-grained teaching (MgT), the student has improved consistently, obtaining better SumR, see Setup\#7 (199.8, taught by X-CLIP), Setup \#11 (199.4, taught by TS2-Net), and Setup \#12 (200.1, taught by X-Pool). Comparing the performance of a specific teacher and its student, we see a clear pattern that their performance is highly correlated. Better teacher leads to better student. 

We also try a multi-teacher teaching strategy (Setup\#13), where $\ell_{CgT}$ and $\ell_{FgT}$ are computed per teacher and minimized jointly. Compared to its single-teacher counterparts, \ie Setup\#7 and Setup\#11, better performance is obtained, yet with no extra overhead in the retrieval stage.

In addition, we experiment with a stronger backbone, substituting ViT-B/16 for ViT-B/32 as the visual encoder. While both teacher, \ie X-CLIP (ViT-B/16), and student (Setup\#1) are better than their ViT-B/32 counterparts, MgT is again effective, lifting SumR from 201.2 to 207.0. 

%\xr{describe shortlist and explain why X-CLIP is chosen as the default choice}

%We select X-Pool, X-CLIP, and TS2-Net as the teachers, as they are  different structures and perform well on the T2VR task. We also choose X-CLIP (ViT-B/16) as a teacher because it uses different initialization weights CLIP (ViT-B/16). All these methods support the computation of both coarse-grained and fine-grained relevance scores.  Meanwhile, the sufficient variability suggests that the proposed approach is not reliant on any specific teacher. For our ablation study, we choose X-CLIP as the primary teacher because it's relatively stable and available across multiple datasets.




\input{tables/ablation.tex}

% \input{iccv2023AuthorKit/tables/ab_student.tex}
% \input{iccv2023AuthorKit/tables/ab_loss.tex}
% \input{iccv2023AuthorKit/tables/ab_fineloss.tex}
% \input{iccv2023AuthorKit/tables/ab_vit16.tex}
% \input{iccv2023AuthorKit/tables/ab_multi}

%\medskip

\textbf{Choice of the student network}. The better performance of Setup\#2 against Setup\#0 (196.3 versus 195.5) indicates that the AFA module is helpful, even under regular training. Further, we compare CLIP4Clip and CLIP4Clip+AFA in the coarse-grained teaching (CgT) mode, see Setup\#3 and Setup\#4. The latter has higher SumR of 198.0. Our choice of using CLIP4Clip+AFA as the student network is verified.
% In what follows, we use CLIP4Clip+AFA as the student network.

%\textbf{Stronger student networks}. Using CLIP4Clip as a baseline student network, we inserted an $AFA$ module to create a stronger student network: CLIP4Clip+AFA. In Tab.\ref{table:ablation}, we can observe that CLIP4Clip+AFA has superior performance than CLIP4Clip 0.8 SumR (\#2 vs \#0). This performance improvement is attributed to the self-attention mechanism of the $AFA$ module, which assigns different weights to different frames. Additionally, another advantage is that the $AFA$ module provides an interface for frame importance, which can be taught by teacher models. We also provide an CLIP4Clip(ViT-B/16) for later comparison.

\textbf{Which loss for CgT}? Comparing Setup\#4 (the Pearson distance loss $d_p$) and Setup\#5 (the Huber loss as previously used by TeachText), the former is marginally better (198.0 versus 197.8). In fact, our experiments on the other datasets show that $d_p$ consistently outperforms the Huber loss. 

%By default, we use the Pearson distance $d_p$. 

\textbf{Is MgT really necessary}?  Setup\#4, Setup\#6 and Setup\#7 correspond to  the student network trained by CgT, by FgT and by MgT, respectively. MgT has SumR of 199.8, followed by CgT (198.0) and FgT (197.3). With MgT, the performance gap between the student (CLIP4Clip+AFA) and the teacher (X-CLIP), measured by the absolute difference of SumR, is reduced from 4.5 to 1.0. The necessity of MgT is verified. 


\textbf{Which loss for FgT}? By default, we use CE as $\ell_{FgT}$. We compare CE with two alternatives, namely $d_p$ and Huber, see Setup\#8 to \#10. CE is the best loss for FgT.

%\textbf{Effectiveness of $\ell_{CgT}$}. When we use X-CLIP as the teacher for coarse-grained teaching, we can see that both CLIP4Clip and CLIP4Clip+AFA achieve \textbf{1.0} (\#3 vs \#0) and \textbf{1.7} (\#4 vs \#2) absolute improvement in SumR, respectively. This indicates that coarse-grained distillation is an effective way to improve the performance of the student models. 



%\textbf{Effectiveness of $\ell_{FgT}$}. CLIP4Clip does not support fine-grained teaching. However, CLIP4Clip+AFA, after fine-grained teaching, performs \textbf{1.0} better than itself without fine-grained teaching in Mean. This indicates that the weight distribution of different frames guided by fine-grained teaching is better than that learned solely by self-attention.




%\textbf{Ablation Study of $\ell_{CgT}$.} Coarse-grained Teaching is knowledge distillation on cross-modal similarity matrixs. To the best of our knowledge, there has been no clear indication of which distillation loss performs better in video-text retrieval tasks. In TeachText\cite{teachtext}, it uses Huber Loss as default disti. We also notice that Pearson Distance is proposed as a measure metric in \cite{peason}. After comparing two losses in Tab.\ref{ab_loss}, Pearson Distance Loss outperforms the other two distance metrics on four datasets. We come to the conclusion that Pearson Distance has a clear advantage in cross-modal retrieval distillation, thanks to its robustness to distribution changes.

% The naive idea is to mimic CLIP4Clip\cite{clip4clip} and use symmetric cross entropy to measure the distance between two similarity matrixs.



%\textbf{Ablation Study of $\ell_{FgT}$.}
%xxx.




%\textbf{Comparison on CLIP(ViT-B/16).} xxx.




%\textbf{Multi-teacher Teaching.} TeachCLIP also leverages multiple teachers with ease. We simply use multiple teachers to conduct Fine-grained and Coarse-grained Teaching for a student at the same time. The advantage of multi-teacher teaching is that it does not increase computational or storage requirements during the student model inference and video-text feature matching. We can still gain the benefits of ensemble learning with multiple teachers and improve the performance of the student model. Referring to Tab.\ref{ab_multi}, it can be observed that the multiple teachers distillation consistently outperforms single teacher distillation on all datasets, which demonstrates the effectiveness of multi-teacher teaching.




\textbf{Qualitative analysis}. Some qualitative results are given in Fig. \ref{fig:vis}. Consider the result at the top for instance. The first frame is the most salient, as it shows key objects, \ie a girl in blue color dress and black shirt man, specified in the query. By computing frame-text relevance on the fly, X-CLIP successfully identifies this frame. For this frame, TeachCLIP also gives a larger weight, albeit precomputed. Similar results can be observed in the other two examples. These qualitative results further confirm the viability of TeachCLIP. 


%To qualitatively validate the effectiveness of our proposed TeachCLIP...


% \begin{figure}[ht!]
% %   \setlength{\abovecaptionskip}{5pt}
%   \centering
%   \includegraphics[width=\columnwidth]{iccv2023AuthorKit/figures/dist.pdf}
%   \caption{\textbf{xx}}
%   \label{fig:dist}
% \end{figure}


\begin{figure*}[ht!]
%   \setlength{\abovecaptionskip}{5pt}
  \centering
  \includegraphics[width=2\columnwidth]{figures/vis.pdf}
  \caption{\textbf{Visualization of video frames,  frame relevance / weights by X-CLIP (teacher),  CLIP4Clip-AFA (student w/o MgT) and TeachCLIP ( student with MgT), and video ranks} (lower rank better). While both students have their frame weights pre-computed in a query-independent manner, the weights by TeachCLIP are more close to the query-dependent weights by X-CLIP, especially on salient frames (manually marked out by red rectangles for the ease of reference). 
  %For each frame displayed above, the corresponding bar plot depicts its frame-wise weight with respect to a specific query. The blue bars indicate the frame weight distribution predicted by the teacher model X-CLIP, while the red and green bars represent the distributions of the student models CLIP4Clip+AFA with and without fine-grained teaching, respectively. 
  %Dataset: MSRVTT-1k.
  }
  \label{fig:vis}
\end{figure*}



==> cvpr2023-author_kit-v1_1-1/algorithm.tex <==
\begin{algorithm}
\caption{TeachCLIP in a PyTorch style}
\label{alg:teachclip}
% \KwIn{$\{(x_i, t_i) |i=1,\ldots,b\}$}
% \KwOut{$G_{s+t}$}


\begin{PythonB}
Input: Training data loader D={(v, t)}
       Trained teacher network
Ouptput: Trained student network

optimizer = torch.optim.Adam(student.parameters)
for e=1,2,..., MAX_EPOCHES:
    for mini-batch {(v, t)} in D:
        optimizer.zero_grad()
        y_c, y_f = teacher({(v, t)}) 
        B, w = student({(v, t)})
        l_CgT = pearson_distance_loss(y_c, B)
        l_FgT = cross_entropy_loss(y_f, w)
        l_IN = symmetric_InfoNCE_loss(B)
        loss = l_CgT + l_FgT + l_IN
        loss.backward()
        optimizer.step()
\end{PythonB}
% # load a mini-batch B of b video-text pairs $\{(x_i, t_i) |i=1,\ldots,b\}$
% def teacher(x, t):
%     return y_c, y_f
% temporal modeling, resulting in m en-
% hanced features
\end{algorithm}


% # b: batch size
% # m: frame number in a video
% # d: feature dimension

% # load a minibatch of b video-text pairs
% for (x,t) in loader:
%     # teacher
%     # y_c: coarse-grained relevance score [b,b]
%     # y_f: fine-grained relevance score [b,m]
%     y_c, y_f = teacher(x,t) 

%     # student
%     # B: similarity matrix [b,b]
%     # w: frame weight [b,m]
%     B, w = student(x,t)

%     # loss
%     l_CgT = pearson_distance_loss(y_c,B)
%     l_FgT = cross_entroy_loss(y_f,w)
%     l_IN = symmetric_infonce_loss(B)
%     loss = l_CgT + l_FgT + l_IN
%     loss.backward()
    
%     # update
%     update(student)

% def student(x, t):
%     # f: frame: [b, m, 224, 224, 3]
%     f = video-to-frames(x)
%     # v: frame feature [b,m,d]
%     v = ViT(f)
%     # phi: temporal enhanced feature [b,m,d]
%     phi = Transformer_4(v) 
%     # w: frame weight [b,m]
%     w = AFA(phi)
%     # video feature [b,d]
%     phi_x = weighted_sum(phi,w)
%     # text feature [b,d]
%     phi_t = GPT-2(t)
%     # similarity matrix [b,b]
%     B = matrix_multiply(phi_x,phi_x.t())
%     return B,w

==> cvpr2023-author_kit-v1_1-1/backup.tex <==


\textbf{Pearson Distance.} 
 The pearson correlation coefficient is used to calculate the cosine similarity of two centered vectors. We define the $\rho _p(\mathbf{a},\mathbf{b})$ as the pearson correlation coefficient between two N-dimension distributions $\mathbf{a}$ and $\mathbf{b}$, which is more robust to distribution changes. The specific formula is as follows:
 
\begin{equation} \label{eq:peasondefine}
\rho_p(\mathbf{a},\mathbf{b})=\frac{\sum_{i=1}^{N}(\mathbf{a}_i-\bar{\mathbf{a}})(\mathbf{b}_i-\bar{\mathbf{b}})}{\sqrt{\sum_{i=1}^{N} (\mathbf{a}_i-\bar{\mathbf{a}})^2 \sum_{i=1}^{N} (\mathbf{b}_i-\bar{\mathbf{b}})^2}}
\end{equation}

Here $\bar{\mathbf{a}}$ and $\bar{\mathbf{b}}$ represent the mean value of $\mathbf{a}$ and $\mathbf{b}$. The Pearson Distance is defined as $d_p(\mathbf{a},\mathbf{b}) = 1-\rho _p(\mathbf{a},\mathbf{b})$.



We use CLIP4Clip\cite{clip4clip} as a baseline student architecture, due to its low computational and offline storage costs. 
On the visual side, it is composed of an frame encoder and temporal encoder module, and the text side is a text encoder module. 
Although it can exploit the sequential information between frames by the temporal encoder, we argue the current architecture design doesn't consider the importance of different frames.
Therefore, we propose a attentional feature aggregation ($AFA$) module to reasonably assign weights for different frames, which is very lightweight and almost doesn't affect the inference speed.

The detailed structure of the $AFA$ is shown in Fig.\ref{fig:structure}.
Starting with the frame-level features $\mathbf{f}$ extracted by CLIP, $\Phi$ is obtained through the temporal encoder module.
We can obtain weights $\mathbf{w}=\{w_1, \ldots, w_m\}$ of different frames by passing $\Phi$ through $AFA$.
The scale operation controls the steepness of the frame weight distribution, which means it is used to balance the same weight for all frames or very high weight for only one frame.
Finally, we sum $\Phi$ with $\mathbf{w}$ as the weight to get video-level features.

\begin{figure}[ht!]
%   \setlength{\abovecaptionskip}{5pt}
  \centering  \includegraphics[width=\columnwidth]{figures/structure}
  \caption{\textbf{The visual feature re-learning module of our CLIP-based text-to-video retrieval network}. The module consists of 4$\times$ Transformer blocks, which exploits inter-frame information to enhance the original frame-level features $\{f_1, \ldots, f_m\}$, and a simple attentional feature aggregation (AFA) block that weightedly combines the frame-level features. AFA, with its produced weights $\{w_1, \ldots, w_m\}$ supervised by a specific teacher network, provides an effective mean for fine-grained knowledge distillation from the teacher network to our network.}
  \label{fig:structure}
\end{figure}



\subsection{Teacher Models} \label{ssec:teacher}


We use XCLIP\cite{xclip} and TS2Net\cite{ts2net} as teacher models, because these two models achieve significantly better performance than CLIP4Clip by fine-grained video text interaction, which brings the increase of computational complexity and offline storage. So we distill these two teachers to make the student model achieve a trade off between performance and efficiency.


Given a batch of $B$ pairs randomly sampled from the dataset, we use the student model to extract video features and text features respectively. 
We calculate the cosine score of a text and video feature as the cross-modal similarity in Eq.\ref{eq:cosine}, where $M(i,j)$ represents the similarity between the i-th text and the j-th video in the similarity matrix.
\begin{equation} \label{eq:cosine}
M(i,j) = \frac{\mathbf{t}_{i}^{T}\mathbf{v}_{j}}{\left \| \mathbf{t}_{i} \right \|\left \| \mathbf{v}_{j} \right \|}
\end{equation}




\noindent $\bullet$  W2VV++\cite{w2vv++} conducts once 2048-dimension floating point vector multiplication for each video-text pair similarity calculations. \\
\noindent $\bullet$ DualE\cite{dualencoding} conducts a video-text similarity calculation based on 2048-dimension vectors. \\
\noindent $\bullet$ CE\cite{ce} conducts 9 video-text similarity calculations in different common space based on 768-dimension vectors.
\noindent $\bullet$ SEA\cite{sea} conducts 5 video-text similarity calculations in different common space based on 2048-dimension vectors. \\
\noindent $\bullet$ MMT\cite{mmt} conducts 7 video-text similarity calculations in different common space based on 512-dimension vectors. \\
\noindent $\bullet$ TeachText\cite{teachtext} conducts a video-text similarity calculation based on 768-dimension vectors. \\
\noindent $\bullet$ CenterCLIP\cite{centerclip} conducts 3$\sim$15 segment-text similarity calculations for each video-text pair based on 512-dimension vectors. \\
\noindent $\bullet$ CLIP4Clip\cite{clip4clip} conducts a video-text similarity calculation based on 512-dimension vectors. \\
\noindent $\bullet$ TS2-Net\cite{ts2net} conducts 12$\sim$64 frame-text similarity calculations for each video-text pair based on 512-dimension vectors. \\
\noindent $\bullet$ X-CLIP\cite{xclip} conducts 1 video-text, 12$\sim$64 frame-text, 32$\sim$64 video-word and 32x12$\sim$64x64 frame-word  similarity calculations for each video-text pair based on 512-dimension vectors. \\
\noindent $\bullet$ X-Pool\cite{xpool} conducts 12 frame-text similarity calculations based on 512-dimension vectors. Then, 12 similarity scores is adjusted to 12 frame weights by softmax. The fusion feature is obtained by performing 12 times of weight-feature dot product and 11 times of feature vector addition. The fusion feature is multiplied by 512x512 matrix to obtain the final video feature. Finally, the video-text similarity calculation based on 512-dimension vectors.


==> cvpr2023-author_kit-v1_1-1/conclusion.tex <==
% For text-to-video retrieval, we propose TeachCLIP that distills knowledge from a relatively heavy teacher to an efficient student through multi-grained teaching. Our experiments show that the student's performance is highly correlated with it's teacher. For more effective knowledge distillation, we introduce a lightweight AFA block for the student network and explore different loss for multi-grained teaching. Finally, we achieve a well trade-off between effectiveness and efficiency for the trained student model.

%In this paper, we present a multi-grained teaching method TeachCLIP for efficient text-to-video retrieval. TeachCLIP distills knowledge from a CLIP-based computationally heavy teacher to an efficient student. Meanwhile, we propose an AFA module to assist the CLIP4clip-based student in distinguishing the importance of frames. We take extensive experiments on four datasets: MSRVTT, MSVD, LATEX, and ActNetCap. TeachCLIP achieves a well trade-off between effectiveness and efficiency and AFA can effectively produce frame-specific weight.

We propose TeachCLIP with multi-grained teaching (MgT) for efficient text-to-video retrieval (T2VR). Extensive experiments on multiple public datasets allow us to conclude as follows.  The performance of the student and the teacher is positively correlated. Better teacher leads to better student. While coarse-grained teaching and fine-grained teaching are helpful even used separately, their joint use, namely MgT, is the best. The overall performance gap between CLIP4Clip (w/o teaching) and X-CLIP is 5.1 in terms of SumR averaged over all test sets. With MgT, the gap is reduced to 1.0. As the student network is designed to have the same efficiency and compactness as CLIP4Clip at the retrieval stage, the much reduced performance gap justifies the viability of the proposed method.

==> cvpr2023-author_kit-v1_1-1/experiment.tex <==

%Motivated by the observation from Fig.\ref{fig:insight}, our work TeachCLIP aims to study how to utilize knowledge distillation to trade off performance and efficiency in the video-text retrieval task. We think that the effect of knowledge distillation depends on the superior limit of teacher, students' ability to receive and carry knowledge, and the specific implementation of knowledge distillation. Our TeachCLIP method is applicable for any teacher. Based on CLIP4Clip, we design a more suitable CLIP4Clip-AFA model as a student. Further, we propose a fine-grained distillation approach to achieve teaching. The architecture of the entire model is shown in Fig.\ref{fig:framework}.

\subsection{Experimental Setup} 

\textbf{Datasets}. We adopt the following public datasets that have been frequently used for T2VR evaluation: 
%To demonstrate the effectiveness and efficiency ability of our method, we perform experiments on the commonly used benchmark text-video retrieval datasets of 
MSRVTT\cite{msrvtt}, MSVD\cite{msvd}, VATEX\cite{vatex} and ActivityNet-Caption (ActNetCap) \cite{activitynet}. While the original data split of MSRVTT has nearly 3k test videos and 60k sentences, Yu \etal suggest another split of 9k videos for training and 1k video-text pairs for testing \cite{msrvtt-1ka}. Probably due to the relatively smaller testset size that makes the evaluation more computation-resource friendly, the 1k edition (MSRVTT-1k) appears to be more popular than its 3k counterpart (MSRVTT-3k). We follow this practice, using MSRVTT-1k as the primary dataset for our ablation study. 

For MSVD, we use its official data slit. For VATEX, we use the split by Chen \etal \cite{hrg}. As for ActNetCap, we adopt the split by Gabeur \etal \cite{mmt}, testing on `val1' as \cite{clip4clip,xclip,ts2net}. Also notice that in contrast the other datasets that use a sentence as a query, ActNetCap, with descriptions per video merged into a paragraph, essentially performs paragraph-to-video retrieval. See \cref{tab:datasets} for an overview.

\input{tables/dataset}



%In the first three datasets, a video matches multiple independent sentences, and a video matches only one sentence in ActivityNet-Caption.

%\textbf{MSRVTT}\cite{msrvtt} includes 10,000 videos and each video contains 20 captions. There are two widely-used splits: "1k" split proposed by \cite{msrvtt-1ka} and the offical "3k" split. Specificly, "1k" adopts 9,000 videos and 180,000 captions for training and utilizes 1,000 video-text pairs as the test set. "3k" has 6,513 videos with its corresponding captions as training set, 497 videos for validating and 2990 videos for test.

%\textbf{VATEX}\cite{vatex} contains 34,991 videos with 10 captions per video.  Following HGR\cite{hrg}’s split, we adopt 25,991, 1,500, and 1,500 videos for training, validating, and test.

%\textbf{MSVD}\cite{msvd} contains 1,970 videos, where each video is annotated with 40 captions. We follow the official data splits: 1,200, 100, 670 videos for training, validating, and test.

%\textbf{ActivityNet}\cite{activitynet} is a dataset for video-paragraph retrieval, consisting of 20,000 YouTube videos where all descriptions are concatenated into one caption. We adopt the evaluation protocol following \cite{multimodal} and report our results on the 'val1' split.


%\subsection{Common Setups} \label{ssec:setup}



\textbf{Evaluation criteria}.
We report standard rank-based metrics, \ie Recall at top $k$ ($k$=1, 5, 10) and SumR (R1+R5+R10) as a combined metric to assess the overall performance of a specific method. 


\textbf{Implementation details}. Subject to our computation capacity ($8\times$ NVIDIA GeForce RTX 3090 24GB GPUs), the default setting is as follows, unless otherwise specified. We use ViT-B/32 as the visual encoder and GPT-2 as the textual encoder, initialized using an OpenAI-released CLIP\footnote{\url{https://github.com/openai/CLIP}}.  In order to reduce the risk of catastrophic forgetting, we empirically set the initial learning rate in a module-specific manner: 1e-7 for ViT-B/32 and GPT-2, and 1e-4 for the remaining modules in a specific network. The network is trained in 10 epochs at maximum by an Adam optimizer \cite{adam}, with the learning rate decayed by a cosine schedule strategy \cite{sgdr}. The input frame size is $224 \times 224$. The maximum length of frame tokens and word tokens are set to 12 and 32, respectively. The mini-batch size is 240, except for ActNetCap, which has much longer videos and texts than the other datasets and thus a smaller batch size of 96 is used. 

For MSRVTT-3k, MSVD and VATEX each of which has a separate validation set,  models maximizing R1 on the validation set are chosen. As for MSRVTT-1k and ActNetCap which has no such validation set, we follow \cite{clip4clip,xclip,ts2net}, reporting peaking performance on the test set. 


%We conduct our experiments on 8 NVIDIA GeForce RTX 3090 24GB GPUs using the PyTorch library. The text encoder and frame encoder parameters are initialized from the public CLIP, and we apply different learning rates to different modules. The text encoder and frame encoder are initialized with an initial learning rate of 1e-7, while other modules start with 1e-4. During the training process of the teacher or student, We optimize networks using The Adam\cite{adam} optimizer and decay the learning rate with a cosine schedule strategy\cite{sgdr}. The dimension of text, frame and video embedding is 512. For the MSRVTT-1k, MSRVTT-3k, MSVD and VATEX, we set the maximum word token length, frame length, batch size and training epoch to 32, 12, 240 and 10. As for ActivityNet, because the text and video duration is longer, we set the maximum word token length, frame length to 64, 64. To accommodate the limitation of GPU memory, we reduce the batch size for ActivityNet to 96. sets. We adopt uniform frame sampling and use ViT-B/32 as the backbone if not specified, with an input image size of 224.  


 %If a validation set is available, we select the model that achieves the best R1 score on the validation set. Otherwise, we select the model based on the test set. 

% During distillation, we set the temperature to 1.0 and the scale parameter to 0.1.




\subsection{Evaluating TeachCLIP} \label{ssec:ablation}

\input{ablation}


\subsection{Comparison with Existing Methods} \label{ssec:performace}


\textbf{Baselines}. We compare with both feature re-learning based methods and CLIP-based end-to-end methods. For the purpose of reproducible research, we include the following peer-reviewed, open-sourced methods: 
\begin{itemize}
    \item \emph{Feature re-learning}: W2VV++\footnote{\url{https://github.com/li-xirong/w2vvpp}}\cite{w2vv++}, DualE\footnote{\url{https://github.com/danieljf24/hybrid_space}}\cite{dualencoding}, CE\footnote{\url{https://github.com/albanie/collaborative-experts}}\cite{ce}, SEA\footnote{\url{https://github.com/li-xirong/sea}}\cite{sea}, MMT\footnote{\url{https://github.com/gabeur/mmt}}\cite{mmt}, TeachText\footnote{\url{https://github.com/albanie/collaborative-experts}}\cite{teachtext}, and LAFF\footnote{\url{https://github.com/ruc-aimc-lab/laff}}\cite{laff}. 
    \item \emph{CLIP-based end-to-end}: Besides CLIP4Clip \cite{clip4clip}, X-CLIP \cite{xclip}, TS2-Net \cite{ts2net} and X-Pool \cite{xpool} that have been evaluated in our ablation study, we include CenterCLIP\footnote{\url{https://github.com/mzhaoshuai/CenterCLIP}}\cite{centerclip}.
\end{itemize}

\input{tables/all_dataset.tex}

\textbf{Effectiveness comparison}. The multi-dataset performance of the varied methods is given in Table \ref{table:alldatasets}. Noticeable performance gap exists between the feature re-learning based methods (the top part of Table \ref{table:alldatasets}) and the CLIP-based end-to-end methods (the bottom part of the same table). The former can be much improved by adding pre-extracted CLIP features (the middle part, cited from \cite{laff}). Consider MMT, for instance. The inclusion of the CLIP feature brings in a clear improvement (SumR 145.7 $\xrightarrow{}$ 186.1 on MSRVTT-1k). Nonetheless, they remain inferior to the end-to-end methods.


Among the end-to-end methods being compared, there is no clear winner that tops the performance on all the five datasets. X-Pool is the best on MSRVTT-1k, CenterCLIP is the best on ActNetCap, whilst X-CLIP leads on MSRVTT-3k and MSVD. Still, our evaluation confirms that X-CLIP has the best overall performance. 

The performance gap between CLIP4Clip and X-CLIP, measured in terms of the absolute difference of their SumR scores per dataset, is as follows: MSRVTT-1k 5.3, MSRVTT-3k 6.6, MSVD 3.5, VATEX 0.0, and ActNetCap 10.0. The overall gap averaged over the datasets is 5.1. 
TeachCLIP, as efficient as CLIP4Clip, reduces the above gap as follows:  MSRVTT-1k 5.3 $\rightarrow$ 1.0, MSRVTT-3k 6.6 $\rightarrow$ 3.3, and ActNetCap 10.0 $\rightarrow$ 4.0. Even more, TeachCLIP (marginally) surpasses X-CLIP on MSVD (210.2 versus 210.1) and VATEX (251.6 versus 248.5). While one would normally not  expect the student to beat the teacher, our interpretation of this counter-intuitive result is as follows. When the teacher and the student have  distinct  network structures yet with close performance, as in the cases of MSVD and VATEX, the teacher may provide complementary information that the student cannot learn by itself. As such, MgT has an effect of ensemble learning to train a better model. In sum, the overall gap is reduced from 5.1 to 1.0. The result justifies the effectiveness of the proposed TeachCLIP method. 

%Considering both performance and efficiency, we compare TeachCLIP with peer-reviewed and open-sourced methods on MSRVTT-1k, MSRVTT-3k, MSVD, VATEX, and ActivityNet. We carefully analyze the computational complexity and storage of these methods, and the analysis process is in the supplementary material. By analyzing the Tab.\ref{table:alldatasets} for the MSRVTT-1k, we gain the following observation.

%\quad$\bullet$  CLIP4Clip and our method both maintain optimal computational and storage efficiency. However, in terms of performance, our TeachCLIP significantly outperforms CLIP4Clip. We obtain \textbf{45.2} R1 (\textbf{+5.6\%} relative improvement, \textbf{+2.4} absolute improvement) and \textbf{199.8} SumR (\textbf{+2.2\%} relative improvement, \textbf{+4.3} absolute improvement).

%\quad$\bullet$ We distill X-CLIP to obtain a student model expressed as TeachCLIP. Compared with X-CLIP, which achieves stable and excellent performance through fine-grained interactions on multiple datasets, our TeachCLIP slightly reduces the performance by \textbf{1.0} absolute SumR. However, for matching one text and video, our TeachCLIP storage space is \textbf{xx} times smaller and our computation is \textbf{xx} times less than X-CLIP. Our method trades off a bit of performance for a significant improvement in efficiency.


%The two points above provide ample evidence that TeachCLIP can improve model performance while maintaining efficiency, which can be attributed to the introduction of our $AFA$ module and the  fine-grained teaching.

%We also further validate the generalization of TeachCLIP on MSRVTT-3k, VATEX, MSVD and ActivityNet in Tab.\ref{table:alldatasets}. We observe that TeachCLIP achieves significant improvements compared to CLIP4Clip, while still maintaining lower computational complexity and storage costs than fine-grained similarity calculation methods.
%Specifically, TeachCLIP outperforms the CLIP4Clip  by \textbf{+3.3} (\textbf{+2.2\%}), \textbf{+3.0} (\textbf{+1.2\%}), \textbf{+3.6} (\textbf{+1.7\%}), \textbf{+3.2} (\textbf{+1.6\%})
%SumR absolute (relative) improvement on aforesaid four datasets respectively. This demonstrates that our proposed TeachCLIP can achieve consistent 
%superior performance under the constraints of computation and storage. More experimental results about the V2TR task are in the supplementary materials.


\textbf{Storage comparison}. Per model, we calculate for a given video all features that are needed at the retrieval stage and can be precomputed. Consider X-CLIP and X-Pool for instance. Frame features are needed for frame-text matching, so they have to be stored. By contrast, CLIP4Clip and TeachCLIP use no frame features for retrieval. Given 4 bytes per floating point, CLIP4Clip and TeachCLIP have the smallest storage footprint of 2KB per video, see the third column of Table \ref{table:alldatasets}.



%没写teachclip

%We calculate the storage space required for each video in the gallery using PyTorch's default floating-point storage method, which uses 32 bits (4 Bytes) per floating-point number. We define 1KB as 1024 Bytes.

%Some methods only require storing a single video feature. For example, the feature dimensions for CLIP4Clip\cite{clip4clip}, TeachText\cite{teachtext}, DualE\cite{dualencoding}, and W2VV++\cite{w2vv++} are 512, 768, 2048, and 2048, respectively, and their corresponding storage spaces are 2KB, 3KB, 8KB and 8KB. Some methods employ a strategy of using multiple common feature spaces, requiring storing multiple features for each video. For instance, CE\cite{ce}, SEA\cite{sea}, and MMT\cite{mmt} require storing 9 768-dimensional feature (27KB), 5 2048-dimensional features (40KB), and 7 512-dimensional features (14KB), respectively.

%CenterCLIP\cite{centerclip} divides a video into multiple segments, with each segment storing a 512-dimension feature. The number of segments in MSRVTT, MSVD and ActNetCap is 3, 3, and 15 respectively, resulting in storage spaces of 6KB, 6KB, and 30KB.
%TS2-Net\cite{ts2net} requires storing a 512-dimensional feature for each frame of a video individually. For ActNetCap, 64 frame features need to be stored, which is 128KB. For other datasets, 12 frame features need to be stored, which is 24KB.
%X-CLIP\cite{xclip} requires storing both a video feature and multiple frame features simultaneously. The number of frames is 64 in ActNetCap and 12 in other datasets, resulting in storage spaces of 26KB and 130KB, respectively.
%When considering only MSRVTT, X-Pool\cite{xpool} needs to store a 512-dimensional feature for each frame, resulting in 24KB of storage space.




% \noindent $\bullet$ W2VV++\cite{w2vv++} uses a 2048-dimension floating point number vector to store a video feature, which utilizes 8KB storage space. \\
% \noindent $\bullet$ DualE\cite{dualencoding} uses a 2048-dimension video feature, which is composed of a 512-dimension concept space feature and 1536-dimension latent space feature.\\
% \noindent $\bullet$ CE\cite{ce} needs to save 9 different common space video features, and the dimension of each space is 768. \\
% \noindent $\bullet$ SEA\cite{sea} needs to save 5 different common space video features, and the dimension of each space is 2048. \\
% \noindent $\bullet$ MMT\cite{mmt} needs to save 7 different common space video features, and the dimension of each space is 512. \\
% \noindent $\bullet$ TeachText\cite{teachtext} uses a 768-dimension floating point number vector. \\
% \noindent $\bullet$ CenterCLIP\cite{centerclip} divides a video into multiple segments, with each segment storing a 512-dimension feature. The number of segments in MSRVTT, MSVD and ActNetCap is 3, 3, and 15 respectively. \\
% \noindent $\bullet$ CLIP4Clip\cite{clip4clip} saves a 512-dimension video feature. \\
% \noindent $\bullet$ TS2-Net\cite{ts2net} needs to save 512-dimension features of each frame in a video. Except for 64 frames stored in the ActNetCap, the rest are 12 frames. \\
% \noindent $\bullet$ X-CLIP\cite{xclip} needs to save a 512-dimension video feature and 512-dimension features for each frame. The frame number is 64 in the ActNetCap and 12 in other datasets. \\
% \noindent $\bullet$ X-Pool\cite{xpool} needs to save 512-dimension features of each frame in a video. 


\textbf{Efficiency comparison}. For model, we measure the number of FLOPs\footnote{\url{https://github.com/Lyken17/pytorch-OpCounter}} required per video-text matching. As shown in the second column of Table \ref{table:alldatasets}, CLIP4Clip and TeachText are the most efficient. 


%Based on the THOP library\footnote{\url{https://github.com/Lyken17/pytorch-OpCounter}}, we calculate the FLOPs consumed by different methods for one retrieval, i.e., matching one video-text pair. We define 1k FLOPs as 1000 FLOPs.


% 对于视频文本只使用一个特征表示的方法，只需要计算两个特征的余弦相似度，考虑到特征已经经过norm，只需要进行两个特征的vector product。根据xx，yy，zz中不同的特征维度，计算量分别是a，b，c。

% To represent video text using only one feature, we can calculate the cosine similarity between two features by taking the vector product of the two features, given that the features have already been normalized. The computation cost for different feature dimensions in xx, yy, and zz is a, b, and c respectively.




% \input{iccv2023AuthorKit/tables/msrvtt1ka.tex}







==> cvpr2023-author_kit-v1_1-1/introduction.tex <==





This paper aims for efficient text-to-video retrieval (T2VR), letting a common user efficiently retrieve specific videos from many unlabeled videos by textual queries. The T2VR task is challenging due to its cross-modal nature: videos and queries have to be encoded into a \emph{semantically}-aligned common feature space for video-text matching \cite{dualencoding}. 

Due to the great success of the Contrastive Language-Image Pre-Training (CLIP) model \cite{clip} in the image domain, we see encouraging efforts on re-purposing CLIP for video-text matching \cite{clip4clip,clip2video,xclip,ts2net,xpool}. As the first work in this line of research, CLIP4Clip \cite{clip4clip} encodes a given video by first using CLIP's visual encoder to extract image features per frame. The frame-level features, enhanced further by stacked Transformer blocks, are aggregated into a video-level feature by mean pooling. The video feature, with a typical dimension of 512, can be computed and stored in advance, making CLIP4Clip efficient for T2VR. Recent methods, \eg X-CLIP \cite{xclip}, TS2-Net \cite{ts2net} and X-Pool \cite{xpool}, improve over CLIP4Clip by considering more fine-grained frame-text similarities. Despite their better retrieval performance on popular benchmarks \cite{msrvtt,msvd}, these models introduce substantial overhead \wrt offline storage and online computation, see Fig. \ref{fig:insight}, putting their scalability for large-scale T2VR into question.



\begin{figure}[t!]
%   \setlength{\abovecaptionskip}{5pt}
  \centering
  \includegraphics[width=\columnwidth]{figures/first_figure.pdf}
  \caption{\textbf{Effectiveness, efficiency and video-feature storage footprint of present-day (CLIP based) text-to-video retrieval models}. Dataset: MSRVTT-1k \cite{msrvtt-1ka}. Backbone: CLIP(ViT-B/32) \cite{clip}. We propose TeachCLIP to strike a good balance between the three factors.}
  \label{fig:insight}
\end{figure}

The research question arises as \emph{how to reduce the performance gap between CLIP4Clip and the latest CLIP-based methods}? 
%In this paper,  we investigate the possibility of improving the retrieval performance as much as possible, without increasing computational or storage costs.
A relatively straightforward approach is to apply knowledge distillation techniques \cite{hinton2015distilling}, which are developed for improving the performance of a student model by transferring dark knowledge from a relatively larger and stronger teacher model to the student. Indeed, there has been good effort on exploiting such techniques for T2VR. TeachText \cite{teachtext} first trains an ensemble of T2VR models with varied textual encoders. The averaged video-text similarity given by the ensemble is then used as soft labels to supervise a specific student network. As TeachText is designed specifically for video-level knowledge distillation, it remains unclear how to effectively pass fine-grained similarities, which are crucial for the teacher's good performance, on to the student?


%like TeachText\cite{teachtext}. It transfers more precise cross-modal information from multiple teachers to a student, which refers to the similarity matrix that contains the relevance between different texts and videos. However, TeachText is a feature re-learning method that does not allow students to finetune parameters from CLIP. 
%Moreover, employing the similarity matrix for supervision means that only the video-text relevance knowledge can be conveyed, while the teacher's inter-frame relevance knowledge in a video can't be transferred. As a result, this distillation process is relatively crude.

On the other hand, the student network itself shall be capable of accepting both video-level and frame-level cross-modal knowledge from the teacher network. Given that CLIP4Clip lacks such capability, a specific module that can be supervised with both video-level and frame-level soft labels is needed. Meanwhile, the module shall not bring in extra storage / computation cost at the retrieval stage. Bearing these in mind, we propose an Attentional frame-Feature Aggregation (AFA) block, see Fig. \ref{fig:framework} for a conceptual diagram. Given a sequence of frame-level features as input, the AFA block produces frame-specific weights, which will be used to aggregate the frame features to a video-level feature.  Note that the block is not new by itself, as similar blocks have been used for fusing diverse video / text features \cite{laff}. What is novel here is that we not only use the attentive weights to weigh the frame features, but also let the weights imitate the frame-text relevance estimated by the teacher network. By doing so, AFA provides a fine-grained learning (teaching) channel for the student (teacher). In our setting, the student and the teacher are both CLIP-based, so the proposed method is coined \texttt{TeachCLIP}.

%We introduce TeachCLIP: a multi-grained teaching method to implement efficient retrieval. It consists of two parts, namely, coarse-grained teaching and fine-grained teaching.  In particular, Coarse-grained Teaching aims to make a lightweight feature matching student mimic fine-grained feature matching teachers by ditilling the cross-modal similarity matrix. Fine-grained Teaching conveys the importance of different frames to the student by using the similarity between text and different frames as guidance.  To enable the student to learn the importance of different frames, we design an Attentional frame-Feature Aggregation ($AFA$) module. This module can learn the importance by itself even without fine-grained teaching.

In sum, our main contributions are as follows:
\begin{itemize}
    \item We present a first study on reducing the performance gap between CLIP4Clip and the latest CLIP-based methods for efficient T2VR.
    \item We propose TeachCLIP with multi-grained teaching to let a CLIP4Clip based student network to learn from more advanced yet computationally heavy models such as X-CLIP, TS2-Net and X-Pool. In particular, we add the AFA block to CLIP4Clip, which by design introduces no extra storage / computation overhead at the retrieval stage.
    \item Extensive experiments on multiple datasets, \ie MSRVTT-1k \cite{msrvtt-1ka}, MSRVTT-3k \cite{msrvtt}, MSVD \cite{msvd}, VATEX \cite{vatex} and ActNetCap \cite{activitynet}, justify the viability of the proposed method. 
\end{itemize}

%(1).We propose a multi-grained teaching method: TeachCLIP. Coarse-grained Teaching supervise the student network with video-level soft labels predicted by the teacher network. Fine-grained Teaching imparts frame relevance information to student. (2).We design an $AFA$ module, which endows a student model (e.g., CLIP4Clip used in the paper) with the ability to learn the importance of different frames. (3).We validate the effectiveness and efficiency of our method on multiple datasets (MSRVTT, MSVD, VATEX, ActNetCap), with different teachers (X-CLIP, TS2-Net, X-Pool) and based on different backbones (ViT-B/32, ViT-B/16).


% 第一段
% In this paper, we want to study是否能在不增加计算与存储消耗的同时，尽可能提高模型检索性能。
% 一个朴素想法是类似于teachtext，通过知识蒸馏传授给学生更为精准的跨模态信息，这里指蕴含不同文本与视频的相关性的跨模态相似度矩阵，在T2VR任务中。
% 但是teachtext是一种特征重学习方法，他的学生无法实现对于CLIP的权重的调整，此外只使用了相似度矩阵监督学生，意味着只能传递文本与视频的相关性知识，老师中对于视频其他知识的理解无法传递，这样的蒸馏是比较粗糙的。
% 受到X-CLIP,TS2-Net等方法的启发，既然不同帧的在视频文本检索过程中发挥着不同的作用，我们希望能将老师中不同帧的重要性这一关键知识通过蒸馏传授给学生。

% 第二段
% We introduce TeachCLIP: a multi-grained teaching method to implement efficient retrieval. 
% TeachCLIP算法由两部分组成，分别是Coarse-grained Teaching和Fine-grained Teaching。具体来说，粗粒度教学使用pearson距离最小化老师与学生的相似度矩阵。而细粒度教学，是指将文本与不同帧的相似度做为教师指导信息，传授给学生学习不同帧的重要性。
%而为了使得学生具备学习不同帧重要性的能力，我们设计了一个Attentional frame-Feature Aggregation (AFA)模块。这个模块即使在没有细粒度教学的情况下也能进行self-attention,学习不同帧的重要性。


% 第三段
% Our main contributions can be summarised as follows：
% 1.我们提出了一个Multi-Grained Teaching method：TeachCLIP， % 

% 2. 我们设计了一个AFA模块，该模块给学生模型(比如文中使用的CLIP4Clip)提供了可以学习不同帧权重的能力。


% 3. 我们在多个数据集(MSRVTT,MSVD,VATEX,ActNetCap)，不同老师(X-CLIP,TS2-Net,X-Pool)，不同backbone(ViT-B/32,ViT-B/16)的情况下，验证了我们方法的有效性。




% TeachCLIP: a knowledge distillation method for Text2Video retrieval models.

% 我们提出了TeachCLIP, 通过知识蒸馏的方法在尽可能保持性能优秀的同时，很大程度减少了离线计算量与存储空间。在视频文本检索领域领域，我们通常将老师的跨模态相似度矩阵蒸馏给学生，而跨模态的相似度由视频与文本的表征计算得到。在这个创新地提出更为细粒度的知识蒸馏, 通过让学生学习不同帧的重要程度，优化视频特征的表达，进而提高蒸馏的效果。




==> cvpr2023-author_kit-v1_1-1/method.tex <==

\begin{figure*}[t!]
%   \setlength{\abovecaptionskip}{5pt}
  \centering  
  \includegraphics[width=2\columnwidth]{figures/framework.pdf}
  \caption{\textbf{Proposed \textit{TeachCLIP} method for training a video CLIP for efficient text-to-video retrieval}. Given a sequence of frame-level features as input, the AFA block produces frame-specific weights $\{w_1, \ldots, w_m\}$, used to aggregate the frame features to a video-level feature.  Meanwhile, by letting the weights imitate the frame-text relevance $\{y_f(f_1,t), \ldots, y_f(f_m,t)\}$ provided by the teacher network, AFA provides a fine-grained learning (teaching) channel for the student (teacher). The student network is end-to-end trained by jointly minimizing a coarse-grained teaching loss $\ell_{CgT}$, a fine-grained teaching loss $\ell_{FgT}$ and a regular training loss $\ell_{IN}$.}
  \label{fig:framework}
\end{figure*}



\subsection{Problem Setup} \label{ssec:setup}

The setup of this research is as follows.  We are provided with two sorts of CLIP-based T2VR models. The first sort,  using exclusively video-level features for video-text matching, is efficient in terms of storage footprint and retrieval speed. Meanwhile, the other sort, relying on fine-grained cross-modal matching, is more accurate than the former. Such an advantage, however, comes at the cost of substantially increased storage and computation overhead. Viewing the former as a student and the latter as a teacher, the proposed TeachCLIP method aims to improve the relatively weaker student with multi-grained dark knowledge from the teacher, see Fig. \ref{fig:framework} for a conceptual diagram. In what follows, we detail the student network in Sec. \ref{ssec:student}, which will be trained by the proposed multi-grained teaching algorithm in Sec. \ref{ssec:mgt}.



%\textbf{Problem Description.} In the T2VR, task, a dataset is usually composed of paired texts and videos.  We are given a query text and a candidate video set, the target is to rank all videos based on their similarity to the query text. So the difficulty of the problem is how to measure the similarity between a text and video . 
% $t \in \mathcal{T}$
% $v \in \mathcal{V}$
% $\mathcal{T}$ 
%  $\mathcal{V}$

%\textbf{Visual and Text Features.} Following \cite{clip4clip}, we use CLIP image encoder (ViT architecture) as the frame encoder, due to its strong downstream performance. We define a video consists of $m$ frames in chronological order. Frame-level features is denoted as $\mathbf{f}=\{f_1, \ldots, f_m\}$.  A temporal encoder is following the frame encoder to embed  temporal information for the frame-level features and we define the features after the temporal encoder as  $\Phi=\{\phi_1, \ldots, \phi_m\}$.  The temporal encoder is consists of 4 standard transformer blocks. We merge the frame encoder and  temporal encoder together and call it visual encoder. Finally, we obtain the video feature $\mathbf{v}$ by fusing $\Phi$. On the other hand, we also use CLIP text encoder (GPT-2 architecture) as our text encoder. We extract the text feature $\mathbf{t}$ by the text encoder.




% \textbf{Knowledge Distillation.} We use the $\mathbf{T}$ and  $\mathbf{S}$ to represent teacher and student models.


\subsection{The Student Network} \label{ssec:student}

Our student network is based on CLIP4Clip \cite{clip4clip}. Given a video $x$ represented by a sequence of $m$ frames $\{f_1, \ldots, f_m\}$, CLIP4Clip first feeds the frames in parallel into the visual encoder of CLIP, \ie a Vision Transformer (ViT), producing an array of frame-level features $\{v_1, \ldots, v_m\}$, sized $m \times d$.  These features, appended with position encoding, then go through four stacked Transformer blocks for temporal modeling, resulting in $m$ enhanced features $\{\phi_1, \phi_2, \ldots, \phi_m\}$. The video feature $\phi(x)$ is obtained by mean pooling over the enhanced features. As aforementioned, mean pooling, treating the individual frames equally, leads to the performance gap between CLIP4Clip and  recent methods (X-CLIP, TS2-Net, X-Pool \etc) that calculate fine-grained cross-modal similarities. 

We improve CLIP4Clip by replacing its mean pooling layer with an Attentional frame-Feature Aggregation (AFA) block. Given $\{\phi_1, \phi_2, \ldots, \phi_m\}$ as its input, AFA is designed to produce an $m$-dimensional nonnegative weight vector $\{w_1, \ldots, w_m\}$, where $w_i$ shall reflect the importance of frame $f_i$. More formally, the key data flow of the visual side of the student network is expressed as follows:
\begin{equation}
\left\{ \begin{array}{ll}
 \{f_1, \ldots, f_m\} & \leftarrow \mbox{video-to-frames}(x),\\
 \{v_1, \ldots, v_m\} & \leftarrow \mbox{ViT}(\{f_1, \ldots, f_m\}),\\
 \{\phi_1, \ldots, \phi_m\} & \leftarrow \mbox{Transformers}\times4(\{v_1, \ldots, v_m\}),\\
 \{w_1, \ldots, w_m\} & \leftarrow \mbox{AFA}(\{\phi_1, \ldots, \phi_m\}), \\
  \phi(x) & \leftarrow  \sum_{i=1}^m w_i \phi_i.
       \end{array} \right.
\end{equation}

As illustrated in \cref{fig:framework}, we implement the AFA block with a linear layer of $d\times d$, followed by ReLU, another linear layer of $d\times 1$, and finally a softmax layer. As such, the amount of extra parameters introduced by AFA is $O(d^2)$. Such  computational overhead is ignorable. More importantly, AFA provides a fine-grained learning path for the student network, as we will see shortly in \cref{sssec:fgt}. 





\subsection{Multi-grained Teaching} \label{ssec:mgt}

%总所周知，正常的知识蒸馏由两部分，一部分是学生模型与预测结果与GT之间的Loss，另外一部分是老师预测结果与学生预测结果的Loss。

The proposed multi-grained teaching (MgT) algorithm follows a standard SGD procedure. Per training iteration, a mini-batch $B$ of $b$ video-text pairs $\{(x_i, t_i) |i=1,\ldots,b\}$ is randomly sampled from a given training dataset. Such randomness allows us to consider each video  irrelevant \wrt other texts and vice versa within the batch. To simplify our notation, we re-use $B$ as a $b\times b$ video-text similarity matrix derived from the batch by the student network. More specifically, we have $B_{i,j}$ as the cosine similarity between $\phi(x_i)$ and $\phi(t_j)$, $i,j=1,\ldots,b$. Accordingly, the $i$-th row $B_{i,\cdot}$ stores similarity scores of video $x_i$ \wrt all $b$ texts in the batch, while the $j$-th column $B_{\cdot,j}$ stores similarity scores of all $b$ videos \wrt text $t_j$. 

In order to perform MgT, we require two outputs from the teacher network concerning video $x_i$ and text $t_j$. That is, a coarse-grained relevance score of $x_i$ \wrt $t_j$, denoted by $y_c(x_i,t_j)$, and a fine-grained relevance score per frame, denoted by $y_f(f_{i,k},t_j)$, $k=1,\ldots,m$. Note that $y_c$ and $y_f$ can be obtained with ease from the SOTA models such as X-CLIP and TS2-Net that compute both frame-level and video-level relevance scores. Moreover, we assume that $\{y_f(f_{i,k},t_j)\}$ have been softmax-adjusted.

\subsubsection{Coarse-grained Teaching}

Coarse-grained teaching is to supervise the student network with video-level soft labels predicted by the teacher network. To that end, TeachText \cite{teachtext} uses the element-wise Huber loss, enforcing $B_{i,j}$ to be close to $y_c(x_i, t_j)$. However, recent research on knowledge distillation \cite{peason} suggests such type of loss is suboptimal, as enforcing a student model to replicate the output of a much stronger teacher model would unnecessarily increase the difficulty of knowledge distillation and consequently impede transferring truly useful knowledge from the teacher to the student. Instead, \cite{peason} suggests to minimize the Pearson's distance $d_p$ (or equivalently maximize Pearson correlation coefficient), which is known to be invariant under separate changes in scale and location in two given variables.  We consider such invariance also desirable in the current task, as minimizing $d_p$ between the output of the student and the teacher networks is adequate for the student to rank-wisely imitate the teacher. Following this thought, we opt to use $d_p$ as the coarse-grained teaching loss $\ell_{CgT}$. In particular, the loss for video $x_i$ is computed as $d_p(\sigma(B_{i,\cdot}), \sigma(y_c(v_i, \cdot)))$, where $\sigma$ is softmax. In a similar manner, the loss for text $t_j$ is calculated as $d_p(\sigma(B_{\cdot, j}), \sigma(y_c(\cdot, t_j))$. Accordingly, $\ell_{ct}$ is defined as the following batch-level symmetric loss:
%
%use for the following symmetric $d_p$ as the loss for coarse-grained teaching $\ell_{ct}$:
%
\begin{equation} \label{eq:loss-cgt}
\begin{array}{ll}
 \ell_{CgT}  := & \frac{1}{b} \sum_{i=1}^b d_p(\sigma(B_{i,\cdot}), \sigma(y_c(v_i, \cdot)) + \\ 
 & \frac{1}{b} \sum_{j=1}^b d_p(\sigma(B_{\cdot, j}), \sigma(y_c(\cdot, t_j)) ). 
\end{array}
\end{equation}


\subsubsection{Fine-grained Teaching} \label{sssec:fgt}

Recall that at the visual side of the student network, we introduce a lightweight AFA  block to produce $m$ attention weights $\mathbf{w}=\{w_1, \ldots, w_m\}$ for convex combination of the $m$ temporally enhanced frame-level features $\{\phi_1, \ldots, \phi_m\}$. Instead of letting the network learn the weights all by itself, we propose to guide the weights-related learning process with fine-grained relevance information from the stronger teacher network. Intuitively, a frame that is more relevant \wrt the given text shall be weighed more. We therefore compute a fine-grained teaching loss $\ell_{FgT}$ per relevant video-text pair $(v_i, t_i)$ as the cross entropy (CE) loss between the weights and the teacher provided frame-text similarities. A batch-level loss is thus obtained by averaging over all the $b$ relevant pairs in the given batch, namely
\begin{equation} \label{eq:loss-fgt}
\ell_{FgT} := -\frac{1}{b}\sum_{i=1}^b \sum_{k=1}^m y_f(f_{i,k}, t_i) \log w_{i,k}.
\end{equation}

Notice that we do not consider fine-grained teaching on the textual side, \eg exploiting video-word similarities to attentively aggregate word-level features. Our main concern is that in contrast to a keyframe that represents the video content to a large extent, a keyword token alone is largely insufficient to represent the corresponding sentence. Indeed, our preliminary experiment showed that adding an AFA on the textual side brings no improvement. We therefore did not go further in that direction. Following CLIP4Clip, we adopt CLIP's textual encoder, \ie a GPT-2, without changing its network structure. 

%In Sec.\ref{ssec:student}, our proposed $AFA$ module can weight different frames, but the weight is learned by the module itself. Therefore, it is natural to think of supervising weight learning with the help of teachers' guidance. We apply softmax to the similarity vector, which is calculated by the teacher between text and different frame-level features, as the frame-wise relevance score: $\mathbf{y}^{f} = \{ y^{f}_{1},\ldots, y^{f}_{m} \}$. Combined with the $\mathbf{w}$ from the student $AFA$ model, we build a frame-level supervising loss $\ell_{ft}$ (see Eq.\ref{eq:lossfine}) to achieve more fine-grained teaching.
%\begin{equation} \label{eq:lossfine}
%\ell_{ft} = -\sum_{i=1}^{B}\sum_{j=1}^{m}y^{f}_{i,j} \log w_{i,j}
%\end{equation}

In addition to $\ell_{CgT}$ and $\ell_{FgT}$, we calculate the symmetric InfoNCE loss over the similarity matrix $B$. Denoted as $\ell_{IN}$, this loss is commonly used for training cross-modal matching networks \cite{xclip,ts2net,clip4clip,centerclip}. The student network is trained to minimize the sum of the three losses, \ie $\ell_{CgT} + \ell_{FgT} + \ell_{IN}$, with the first two terms responsible for MgT and the last term for regular training. TeachCLIP is easy to implement, see Algorithm \ref{alg:teachclip}.

%for a PyTorch-style algorithm description.
%acts as regular training.  



%The Ground Truth (GT) is a $B$-dimension identity matrix. We construct a cross entropy loss over the similarity matrix as the T2VR loss to train the student model in Eq.\ref{eq:retrievalt2v}. 

%\begin{equation} \label{eq:retrievalt2v}
%\ell_{t2v} = -\frac{1}{B}\sum_{i=1}^{B}log\frac{\exp(M(i,i))}{\sum_{j=1}^{B} \exp(M(i,j))}
%\end{equation}

%Generally, in order to better realize cross-modal matching, we also need a video-to-text retrieval (V2TR) loss $\ell_{v2t}$ based on transpose of $M$. The retrieval loss $\ell_{gt}$ can be formulate as:
% \begin{equation} \label{eq:retrievalv2t}
% \mathcal{L}_{v2t} = -\frac{1}{B}\sum_{i=1}^{B}log\frac{\exp(M(i,i))}{\sum_{j=1}^{B} \exp(M(j,i))}
% \end{equation}

%\begin{equation} \label{eq:retrievalloss}
%\ell_{gt} = \ell_{t2v} + \ell_{v2t}
%\end{equation}

%粗粒度蒸馏
%Let the student imitate the teacher on the cross-modal  similarity matrix, so as to achieve the transfer of dark knowledge. We call it Coarse-grained Teaching. To represent matrix $M$ in a more compact form, we express it as B vectors arranged in rows : $M=\{\mathbf{m}_1, \ldots, \mathbf{m}_B\}$. The teacher's supervised similarity matrix is denoted by $Y^{c}=\{ \mathbf{y}^c_1, \ldots, \mathbf{y}^c_B\ \}$. Inspired by \cite{peason}, we use Pearson Distance to each row of the teacher and student similarity matrix.

%\begin{equation} \label{eq:dist2v}
%\ell_{t2v}^{ct} = \frac{1}{B}\sum_{i=1}^{B}d_p(softmax(\mathbf{m}_i),softmax(\mathbf{y}^c_i))
%\end{equation}

%Similarly, we need to construct a loss $\ell_{v2t}^{ct}$  for the V2TR task based on the transpose of $M$ and $Y^{c}$. The Coarse-grained Teaching loss $\ell_{ct}$ can be formulate as:

%\begin{equation} \label{eq:dis}
%\ell_{ct}=\ell_{t2v}^{ct}+\ell_{v2t}^{ct}
%\end{equation}



% Next, we need to calculate the teacher's similarity matrix $M^{\mathbf{T}}$, and let the student imitate the teacher, so as to achieve the transfer of dark knowledge. Inspired by \cite{peason}, we increase the pearson correlation of two similarity matrixs, where the pearson correlation centers distributions(see Eq.\ref{eq:pearson1},\ref{eq:pearson2}) and makes it more robust to changes. We define  $\sigma(\pi,dim)$ as a softamx function, $\pi$ as a hyperparameter temperature to adjust the distribution and $dim$ as the axis to operate.

% \begin{equation} \label{eq:pearson1}
% \bar{M}(i,j) = \sigma(M(i,j),\pi,1) - \frac{1}{B}\sum_{j=1}^{B}\sigma(M(i,j),\pi,1)
% \end{equation}
% \begin{equation} \label{eq:pearson2}
% \tilde{M}(i,j) = \sigma(M(i,j),\pi,0) - \frac{1}{B}\sum_{i=1}^{B}\sigma(M(i,j),\pi,0)
% \end{equation}

%  We realize the distillation as the following:


% \begin{equation} \label{eq:dist2v}
% \mathcal{L}_{dist2v} = 1-\sum_{i=1}^{B} \frac{\sum_{j=1}^{B}\bar{M}^{\mathbf{T}}(i,j)*\bar{M}^{\mathbf{S}}(i,j)}{\sqrt{\sum_{j=1}^{B}\bar{M}^{\mathbf{T}}(i,j)^2}\sqrt{\sum_{j=1}^{B}\bar{M}^{\mathbf{S}}(i,j)^2}}
% \end{equation}
% % \mathcal{L}_{dist2v}=-\frac{1}{B^2}\sum_{i=1}^{B}\sum_{j=1}^{B}\sigma(\bar{M}^{\mathbf{T}}(i,j),\pi)\log \sigma(\bar{M}^{\mathbf{S}}(i,j),\pi)

% \begin{equation} \label{eq:disv2t}
% \mathcal{L}_{disv2t} = 1-\sum_{j=1}^{B} \frac{\sum_{i=1}^{B}\tilde{M}^{\mathbf{T}}(i,j)*\tilde{M}^{\mathbf{S}}(i,j)}{\sqrt{\sum_{i=1}^{B}\tilde{M}^{\mathbf{T}}(i,j)^2}\sqrt{\sum_{i=1}^{B}\tilde{M}^{\mathbf{S}}(i,j)^2}}
% \end{equation}

% \begin{equation} \label{eq:dis}
% \mathcal{L}_{distill}=\mathcal{L}_{dist2v}+\mathcal{L}_{disv2t}
% \end{equation}
% % the Pearson correlation has an additional shift-invariance by centering the vectors first (see Eq.(7)), and it could be more robust to the distribution changes.
% %realize xx to 
  
%精细化蒸馏



%Three losses merge to guide TeachCLIP learning.

%\begin{equation} \label{eq:teachclip}
%\ell =\ell_{gt} + \ell_{ct} + \ell_{ft}
%\end{equation}



% , where the softmax function is used to generate the distribution of $m$ frames, and $\rho$ is used to scale. Since the vector has only one  axis, the axis is set to 0.
%这里softamx函数用于生成m帧的分布，以及xx用于进行scale。
% \begin{equation} \label{eq:teacherweight}
% \mathbf{w}^{\mathbf{T}} = \sigma((\mathbf{f}^{\mathbf{T}})^{T}(\mathbf{t}^{\mathbf{T}}),\rho)
% \end{equation}

%结合从学生模型中输出的WS，我们构建了frame级别的监督损失Lfine，实现了更加细粒度的蒸馏。



% In this section, we elaborate our proposed TeachCLIP. We first describe in Sec.\ref{ssec:problem} how to train a Video-Text Retrieval model.  In Sec.\ref{ssec:coarse-knowledge}, we exploit the coarse-grained distillation method in different manners. In Sec.\ref{ssec:fine-knowledge}, we 
% innovatively put forward fine-grained knowledge distillation.


% \subsection{Video-Text Retrieval} \label{ssec:problem}
% Let ${ \left \{  (c_{i},v_{i})  \right \} }_{i=1}^{n}$ be a dataset of paired texts and videos. 
% A video $v$ is composed of $m$ frames. %$\{ v^{j} \}_{j=1}^{m}$. 
% We use CLIP as the backbone network structure, due to its strong downstream performance.
% We use $\psi,\phi,\rho$ to indicate the CLIP text encoder, CLIP frame encoder and frame aggregation function.
% Given a set of $B$ pairs randomly sampled from th dataset. Specifically, take the i-th pair as an example.
% Based on the CLIP frame encoder, we can get the frame feature $F_{i} = [\phi(v^{1}_{i}),\phi(v^{2}_{i}),...,\phi(v^{m}_{i})] \in  \mathbb{R}^{m\times d}$, and input it into the frame aggregation function to further obtain the video feature, see Eq.\ref{eq:fusion}.


% \begin{equation} \label{eq:fusion}
% V_{i} = \frac{1}{m}\sum_{j=1}^{m} \rho(F_{i}) \in  \mathbb{R}^{ d}. 
% \end{equation}

% On the text side, we get $C_{i} = \psi(c_{i}) \in  \mathbb{R}^{ d} $ by the CLIP text encoder. 
% When we measure the cross-modal distance score between the i-th text and the j-th video, it is computed by the cosine similarity between the video feature and text feature, see Eq.\ref{eq:cosine}.


% \begin{equation} \label{eq:cosine}
% M(i,j) = \frac{\mathbf{t}_{i}^{T}\mathbf{v}_{j}}{\left \| \mathbf{t}_{i} \right \|\left \| \mathbf{v}_{j} \right \|}
% \end{equation}

% Following \cite{clip4clip}, we use a symmetric cross entropy loss over the similarity matrix to train the model.

% \begin{equation} \label{eq:retrievalt2v}
% \mathcal{L}_{t2v} = -\frac{1}{B}\sum_{i=1}^{B}log\frac{\exp(M(i,i))}{\sum_{j=1}^{B} \exp(M(i,j))}
% \end{equation}

% \begin{equation} \label{eq:retrievalv2t}
% \mathcal{L}_{v2t} = -\frac{1}{B}\sum_{i=1}^{B}log\frac{\exp(M(i,i))}{\sum_{j=1}^{B} \exp(M(j,i))}
% \end{equation}

% \begin{equation} \label{eq:retrievalloss}
% \mathcal{L}_{retrieval} = \mathcal{L}_{t2v} + \mathcal{L}_{v2t}
% \end{equation}




% % $F_{i} = [\phi(v^{1}_{i}),\phi(v^{2}_{i}),...,\phi(v^{m}_{i})] \in  \mathbb{R}^{m\times d}$ 
% % $C_{i} = \psi(c_{i}) \in  \mathbb{R}^{ d} $
% % $V_{i} = \rho(F_{i}) \in  \mathbb{R}^{ d}$
% % $S(i,j) = C_{i}^{T}V_{j}$




% \subsection{Coarse-grained Knowledge Distillation} \label{ssec:coarse-knowledge}
% In a standard knowledge distillation process, the student is improved by the teacher’s predictions and ground truths, where the teacher is trained with supervision.

% Teacher:$\mathcal{T}$ Studnet$\mathcal{S}$


% \subsection{Fine-grained Knowledge Distillation} \label{ssec:fine-knowledge}


\input{algorithm}

==> cvpr2023-author_kit-v1_1-1/related.tex <==

At a high level, 
our idea of multi-grained teaching can be %conceptually 
viewed as knowledge distillation from a relatively heavy teacher network to an efficient student network. Hence, we briefly review progress in T2VR and knowledge distillation, accordingly interpreting our novelty in such a joint context.

%\textbf{Progress on T2VR}. 

\subsection{Text-to-Video Retrieval} \label{ssec:related-video}


\textbf{Effective T2VR}. The majority of the literature is on effectiveness, aiming for better cross-modal matching networks that compute video-text similarity more accurately. Depending on whether video / text feature extractors are trained together with the cross-modal matching module, we categorize existing works into two groups. That is, feature re-learning methods and (CLIP based) end-to-end methods.

Feature re-learning methods typically employ pretrained 2D-CNNs for  \cite{w2vv++,dualencoding}, 3D-CNNs \cite{je,ce} or their combinations \cite{mmt,laff} to obtain an initial feature representation of a given video. Similarly, a given text is encoded either by nontrainable bag-of-words \cite{w2vv++} or by pre-trained text encoders including Word2Vec \cite{w2vv}, BERT \cite{w2vvpp-bert}, GPT \cite{teachtext}, \etc.  Feature re-learning is then performed to project the video and text features into a common latent space, wherein the video-text relevance can be measured in terms of their distance in the common space. While there is still room for improvement, \eg by adding more features with novel feature fusion blocks, see MMT \cite{mmt}, TeachText \cite{teachtext} and LAFF \cite{laff}, the performance of feature re-learning methods is largely bounded by the initial features.  

The advent of CLIP \cite{clip} and its application in the video domain has significantly reshaped the research landscape of T2VR.  CLIP-based end-to-end methods have shown superior performance to their feature re-learning based predecessors on multiple public datasets \cite{clip4clip,ts2net,xpool,xclip}. As an initial attempt in this line of research, CLIP4Clip \cite{clip4clip} employs the visual encoder of CLIP to first extract a sequence of frame-level features. The frame features, updated by a stack of standard Transformer blocks, are averaged to produce a video-level feature. Such a video feature can be precomputed offline, while the storage footprint is linear \wrt the number of videos. Hence, a CLIP4Clip based T2VR system is efficient and compact. Follow-ups of CLIP4Clip, \eg X-CLIP \cite{xclip}, TS2-Net \cite{ts2net} and X-Pool \cite{xpool}, improve video-text matching by fine-grained cross-modal feature interaction and matching. Despite their better performance, local interaction means features used for cross-modal matching have to be computed online, while fine-grained matching results in substantial computation and storage overhead. This puts the scalability of the latest CLIP-based methods into question. 


\textbf{Efficient T2VR}. In order to accelerate video feature extraction, CenterCLIP \cite{centerclip} utilizes a multi-segment token clustering algorithm to find the most representative tokens. Only these essential tokens will be forwarded through the entire Transformers, while those non-essential tokens will be dropped at a pre-specified Transformer block. For video-text relevance estimation, the model requires fine-grained matching at the segment level, making its storage and computation amplified by the number of segments per video. Hence, CenterCLIP remains relatively heavy when compared to CLIP4Clip. We aim for the same efficiency and compactness as CLIP4Clip at the retrieval stage. 

%To that end, the network architecture has to be hacked for token clustering and selection. 


%for segment-level feature extraction \cite{je,ce} 

%Given a query text, the T2VR task aim to retrieve relevant videos from gallery videos. Before the CLIP\cite{clip}, the mainstream T2VR methods are feature-relearning approaches. The sources of the features could be multiple video modalities\cite{je,ce,mmt}, network layers\cite{dualencoding}, and textual modelings\cite{teachtext,w2vv++,sea,laff}. specifically...

%After the emergence of CLIP, the mainstream approaches have gradually shifted towards end-to-end finetuning methods based on CLIP, leading to various derived variants. CLIP4Clip\cite{clip4clip} first proposes multi-frame fusion methods to bridge the gap between image and video modalities, aiming to improve the performance of T2VR. Specifically, the features of each frame are obtained by  CLIP image encoder. These features are then fed into a Transformer model to encode temporal information. Finally, meanpooling is performed on the features to obtain video features, which are used for video-text similarity score calculation with text features from CLIP text encoder.  CenterCLIP\cite{centerclip} proposes multi-segment clustering strategies to split a video into fixed-length segments, and calculates the similarity between text and multiple segment features. The segment-text similarity scores are then averaged to obtain as the video-text similarity score. TS2-Net\cite{ts2net} implements modeling of multi-frame timing by designing a Token Shift module and select one token for each frame as the frame feature.  Multiple frame features are compared with text features to generate frame-text similarity scores, which are then normalized using softmax function to obtain frame weights. Finally, the video-text similarity score is computed as the weighted sum of the frame-text similarity scores. X-Pool\cite{xpool} also considers fine-grained interactions between text and different frame features. Unlike TS2-Net, it combines frame weights with different frame features to form a new video feature. X-CLIP\cite{xclip} is more complex and considers multi-grained contrast of features, including video-sentence, video-word, sentence-frame, and frame-word. Expanding on the foundations of CLIP4Clip, these methods improve performance by more fine-grained similarity calculations, albeit at the expense of increased cost for offline feature storage and online retrieval computation.

% The T2VR task has gained much attention in recent years [7, 10, 21, 22, 25, 36, 49, 53, 60], aiming to retrieve relevant videos by a given query from a set of pre-trimmed video clips. The retrieved clips are supposed to befully relevant to the given query.
% 在CLIP出来之前，主流的T2VR方法是feature-relearnig approaches。
% 得到特征的来源可能是多个视频模态，多个网络层次，以及多种文本建模方式。
% 考虑到本文的不同建模方式，多种文本特征可以用于特征融合再学
 % These methods can be roughly divided into only integrating text features\cite{teachtext,w2vv++,sea}, only integrating video features\cite{je,ce,mmt} and simultaneously integrating features at both ends\cite{laff}. 
% CLIP之后，主流的方法变成基于CLIP的end-end finetuning，并衍生出许多不同的变体。

% We roughly divide the video-text retrieval methods into two categories, feature-fusion approaches and CLIP-based approaches.
% Previous feature-fusion approaches focus on aggregate multiple video or text features. These methods can be divided into only integrating text features\cite{teachtext,w2vv++,sea}, only integrating video features\cite{je} and simultaneously integrating features at both ends\cite{laff}. 
% JE\cite{je} concatenates visual and audio features to fuse video features.
% W2VV++\cite{w2vv++} concatenates three types of text feature vector to form a fused text feature before calculating the similarity with video features. By contrast, SEA\cite{sea} constructs a common space for each type of text feature and then averages the similarities calculated in the individual spaces. TeachText\cite{teachtext} adopts knowledge distillation to ditill multiple common spaces calculated by different text features into one space. LAFF\cite{laff} studies both video-end and text-end feature fusion for video-text retrieval.
% In addition, Dual\cite{dual} tries to integrate the different level features in the model.
% %集成的方法概述

% CLIP\cite{clip} implements the contrastive learning based on a large-scale image-text pairs, which can achieve outstanding cross-modal performance and zero-shot capability. A series of CLIP-based approaches transfer image-text matching to video-text matching.
% %CLIP方法概述

% %根据xx中的定义，这类方法可以分为只集成文本特征，只集成视觉特征和同时集成两端的特征。
% % feature-fusion approaches 目前的



%\subsection{Efficient Text-to-Video Retrieval} \label{ssec:efficient}

% 训练的高效性
% 推理的高效性
% 实时检索的高效性 


% CenterCLIP 



%在视频文本检索的任务中，高效性体现在模型的训练，模型的推理，以及实时检索阶段。
% 如何efficient?

% According to \cite{}, knowledge distillation can be roughly classified into three types: response-based knowledge distillation, feature-based knowledge distillation, and relation-based knowledge distillation.
% Response-based knowledge distillation involves transferring dark knowledge from a teacher to a student by having the student mimic the teacher's logits.
% To fully utilize a teacher's knowledge at different layers of the network, Fitnets\cite{} introduces knowledge distillation based on intermediate features.
% In \cite{}, the method of relational knowledge distillation is proposed, which transfers relations between samples to penalize structural differences.
% 基于响应的知识蒸馏是指让学生在logits上模仿老师的，从而完成darkknowledge的传递。
% 为了充分利用老师模型在网络不同层的知识，
% 知识蒸馏 在 the intermediate features are introduced in Fitnets。
% 借鉴于Relation-Based knowledge distillation上，teachtex, most relevance to our approach, 提出 directly learning the retrieval similarity matrix between the joint query video embeddings in T2VR tasks.
% Of， 在视频文本检索任务重使用了知识蒸馏，具体地。
% 通常我们会使用kl散度作为距离度量，最近也有工作表明pearson距离可以被有效用于知识整理，which can preserve the relative ranks of predictions, instead of aligning the absolute values accurately.




\subsection{Knowledge Distillation} \label{ssec:related-knowledge}

Knowledge distillation is to transfer ``dark'' knowledge from a large, heavily weighted teacher model or ensemble of teacher models to a single, smaller student model, which can be practically deployed \cite{hinton2015distilling}. The form of the knowledge varies, which can be the output of the teacher \cite{peason}, its intermediate representations \cite{fitnets}, or mutual relations of data examples \cite{relation}.  In the context of video-to-video retrieval, DnS is proposed to distill knowledge, represented in the form of video-to-video relevance scores, from a big network to a smaller network \cite{dns}. As for T2VR, TeachText is developed \cite{teachtext}, where a student network is trained to mimic the averaged video-text similarity given by an ensemble of feature re-learning based models. Technically different from DnS and TeachText, the proposed TeachCLIP goes one step further by exploiting intermediate results of an up-to-date CLIP-based model as side information to supervise a CLIP4Clip based student model.

%Gou \etal \cite{kdsurvey} classify existing methods for knowledge distillation into three classes as follows: response-based methods that let the student mimic the teacher's output \cite{pearson} , feature-based methods to let the student mimic the teacher's intermediate representations, and relation-based methods that exploit inter-sample relations to penalize structural differences between the \cite{relation}. 
%Response-based knowledge distillation is to let the student mimic the teacher's prediction.  
%Typically, Kullback-Leibler Divergence is used as the discrepancy metric between a teacher and student. Recently, one work\cite{peason} shows that Pearson Distance can be effectively used for knowledge distillation, which preserves the relative ranks of predictions instead of precisely aligning the absolute values.
%In order to fully utilize the knowledge of a teacher at different layers of the network, Fitnets\cite{fitnets} introduces intermediate features knowledge distillation.

%Relation-based knowledge distillation is proposed in \cite{relation}, which transfers relations between samples to penalize structural differences. Inspired by relation-based knowledge distillation, TeachText\cite{teachtext} proposes directly learning the retrieval similarity matrix from the text-video matching in T2VR tasks.



%\subsection{Comparison to previous approaches} \label{ssec:comparison}

% 在T2VR的方法中，相比于CLIP4Clip，我们在结构上提出了AFA模块使得模型
% 在蒸馏的方法中，对比TeachText仅仅在相似度矩阵上蒸馏，我们提出了多粒度蒸馏，同时进行。

==> cvpr2023-author_kit-v1_1-1/tables/ab_fineloss.tex <==


\begin{table}[ht!]
\caption{\textbf{Ablation study of $\ell_{FgT}$.} Teacher:X-CLIP,Studnet:CLIP4Clip-AFA, $\ell_{CgT}$: Pearson Distance}
\label{ab_loss}
\renewcommand{\arraystretch}{1}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}llllllr@{}}
\hline
 & 1k & \multicolumn{1}{r}{3k} & \multicolumn{1}{r}{VA.} & \multicolumn{1}{r}{MS.} & \multicolumn{1}{r}{Ac.} & Mean \\ \hline
Huber & 199.3 & 154.6 & 250.5 & 209.9 & 197.8 & 202.4 \\
Cross Entropy & 199.8 & 153.4 & 251.5 & 210.2 & 200.1 & 203.0 \\
Pearson & 199.7 & 152.1 & 249.4 & 209.2 & 198.3 & 201.7 \\ \hline
\end{tabular}
}
\end{table}



% \setlength{\tabcolsep}{3pt} % Default value: 6pt
% Default value: 1

==> cvpr2023-author_kit-v1_1-1/tables/ab_loss.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[ht!]
\caption{\textbf{Ablation study of $\ell_{ct}$.}}
\label{ab_loss}
% \setlength{\tabcolsep}{3pt} % Default value: 6pt
\renewcommand{\arraystretch}{1} % Default value: 1
% \centering
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
Distance Metric & 1k & 3k & VA. & MS. & Ac. & Mean \\ \hline
Huber & 197.8 & 150.0 & 247.5 & 205.0 & 180.2 & 196.1 \\
Cross Entropy & 198.2 & 150.6 & 249.3 & 207.0 & 196.5 & 200.3 \\
Pearson & 196.5 & 151.8 & 250.0 & 208.4 & 197.3 & 200.8 \\ \bottomrule
\end{tabular}
}
\end{table}


==> cvpr2023-author_kit-v1_1-1/tables/ab_multi.tex <==

\begin{table}[ht!]
\caption{\textbf{Ablation study of multi-teacher teaching.}}
\label{ab_multi}
% \setlength{\tabcolsep}{1pt} % Default value: 6pt
\renewcommand{\arraystretch}{1} % Default value: 1
% \centering
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lrrrrrr@{}}
\hline
 & 1k & 3k & VA. & MS. & Ac. & Mean \\ \hline
TeachCLIP(TS2Net) & \multicolumn{1}{l}{199.4} & 153.4 & 250.7 & 209.8 & \multicolumn{1}{l}{198.4} & 202.3 \\
TeachCLIP(XCLIP) & \multicolumn{1}{l}{199.8} & 153.4 & 251.5 & 210.2 & \multicolumn{1}{l}{200.1} & 203.0 \\
TeachCLIP(TS2Net,XCLIP) & 201.2 & 154.9 & 251.5 & 210.6 & 201.4 & 203.9 \\ \hline
\end{tabular}
}
\end{table}

% CLIP4Clip & 195.5 & 150.1 & \multicolumn{1}{r}{248.5} & \multicolumn{1}{r}{206.6} & 196.9 & 199.52 \\
% TS2Net & 200.5 & 153.6 & \multicolumn{1}{r}{248.6} & \multicolumn{1}{r}{204.9} & 190.4 & 199.6 \\
% X-CLIP & 200.8 & 156.7 & \multicolumn{1}{r}{248.5} & \multicolumn{1}{r}{209.0} & 204.1 & 203.82 \\

==> cvpr2023-author_kit-v1_1-1/tables/ab_student.tex <==
\begin{table}[ht!]
\caption{\textbf{Ablation study of student network.} We use 1k, 3k, VA., MS., and Ac. to respectively represent the abbreviations of MSRVTT-1k, MSRVTT-3k, VATEX, MSVD, and ActivityNet. The evaluation metric is SumR, and Mean is the average of SumR across multiple datasets.}
\label{ab_student}
% \setlength{\tabcolsep}{1pt} % Default value: 6pt
\renewcommand{\arraystretch}{1} % Default value: 1
% \centering
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lrrrrrrrr@{}}
\toprule
Student network & $l_{ct}$ & $l_{ft}$ & 1k & 3k & VA. & MS. & Ac. & Mean \\ \hline
\multirow{2}{*}{CLIP4Clip} & \ding{55} & n.a. & 195.5 & 150.1 & 248.5 & 206.6 & 194.1 & 199.0 \\
 & \checkmark & n.a. & 196.5 & 151.8 & 250.0 & 208.4 & 197.3 & 200.8 \\ \hline
\multirow{3}{*}{CLIP4Clip-AFA} & \ding{55} & \ding{55} & 196.3 & 152.1 & 249.4 & 208.2 & 194.8 & 200.2 \\
 & \checkmark & \ding{55} & 198.0 & 152.7 & 250.3 & 209.8 & 198.5 & 201.9 \\
 & \checkmark & \checkmark & 199.8 & 153.4 & 251.5 & 210.2 & 200.1 & 203.0 \\ \bottomrule
\end{tabular}
}
\end{table}
% 这里我们使用1k，3k, VA., MS., Ac. 分别代表MSRVTT-1k,MSRVTT-3k,VATEX,MSVD 和ActivityNet的缩写。 衡量指标是SumR，Mean 是多个数据集SumR的平均值。

==> cvpr2023-author_kit-v1_1-1/tables/ab_temp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{\textbf{Ablation study of temperature on MSRVTT-1k.}}
\label{ab_temp}
% \setlength{\tabcolsep}{6pt} % Default value: 6pt
\renewcommand{\arraystretch}{1} % Default value: 1
% \centering
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lrrrr@{}}
\toprule
Temperature & R1 & R5 & R10 & SumR \\ \hline
0.5 & 44.6 & 71.6 & 80.0 & 196.2 \\
1.0 & 44.2 & 71.7 & 80.6 & 196.5 \\
2.0 & 43.3 & 71.0 & 81.3 & 195.6 \\
5.0 & 43.5 & 71.3 & 80.8 & 195.6 \\ \bottomrule
\end{tabular}
}
\end{table}

==> cvpr2023-author_kit-v1_1-1/tables/ab_vit16.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table}[ht!]
% \caption{\textbf{CLIP(ViT-B/16) on MSRVTT-1k.}}
% \label{ab_vit16}
% \renewcommand{\arraystretch}{1} % Default value: 1
% % \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{@{}lrrrr@{}}
% \toprule
% Model & R1 & R5 & R10 & SumR \\ \hline
% CLIP4Clip & 45.4 & 73.5 & 82.3 & 201.2 \\
% X-CLIP & 49.1 & 76.1 & 84.4 & 209.6   \\
% TeachCLIP(X-CLIP) & 48.1 & 75.4 & 83.5 & 207.0 \\ 
% \bottomrule
% \end{tabular}
% }
% \end{table}

 
 
 

 % Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[ht!]
\caption{\textbf{Ablation study of visual encoder on multiple datasets.}}
\label{ab_vit16}
\renewcommand{\arraystretch}{1} % Default value: 1
% \centering
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lrrrrrrrrrrrrrrr@{}}
\toprule
\multirow{2}{*}{\textbf{model}} & \multicolumn{3}{c}{\textbf{MSRVTT-1k}} & \multicolumn{3}{c}{\textbf{MSRVTT-3k}} & \multicolumn{3}{c}{\textbf{MSVD}} & \multicolumn{3}{c}{\textbf{VATEX}} & \multicolumn{3}{c}{\textbf{ActNetCap}} \\
\cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){8-10} \cmidrule(r){11-13} \cmidrule(r){14-16} 
 & R1 & R5 & SumR & R1 & R5 & SumR & R1 & R5 & SumR & R1 & R5 & SumR & R1 & R5 & SumR \\ \hline
 \multicolumn{16}{@{}l}{\textit{ViT-B/32 as visual encoder}:}\\
 CenterCLIP \cite{centerclip} &  44.2 & 71.6 & 197.9 & - & - & -  & 47.3 & 76.8  & 209.7 & - & - & - & 43.9 & 74.6 & 204.3 \\
 CLIP4Clip \cite{clip4clip} & 42.8 & 71.6 & 195.5 & 29.4 & 54.9 & 150.1 & 45.6 & 76.1 & 206.6 & 61.6 & 91.1 & 248.5 & 39.7 & 71.0 & 194.1 \\
X-CLIP \cite{xclip} & 45.3 & 73.7 & 200.8 & 31.2 & 57.4 & 156.7 & 47.2 & 77.0 & 210.1 & 62.2 & 90.9 & 248.5 & 44.4 & 74.6 & 204.1 \\
TeachCLIP(X-CLIP) & 44.0 & 73.5 & 200.1 & 30.4 & 56.3 & 153.4 & 47.4 & 77.3 & 210.2 & 63.6 & 91.9 & 251.6 & 42.2 & 72.7 & 200.1 \\
[3pt]
\multicolumn{16}{@{}l}{\textit{ViT-B/16 as visual encoder}:}\\
CenterCLIP & 48.4 & 73.8 & 204.2 & - & - & - & 50.6 & 80.3 & 219.3 & - & - & - & 46.2 & 77.0 & 210.8 \\
CLIP4Clip & 45.4 & 73.5 & 201.2 & 31.3 & 56.9 & 155.6 & 47.1 & 77.9 & 211.4 & 64.7 & 92.1 & 253.3 & 40.3 & 71.6 & 195.1 \\
X-CLIP & 49.1 & 76.1 & 209.6 & 33.4 & 59.3 & 162.0 & 48.2 & 78.7 & 213.8 & 65.8 & 92.5 & 254.7 & 44.8 & 74.2 & 204.5 \\
TeachCLIP(X-CLIP) & 48.1 & 75.4 & 207.0 & 32.8 & 58.9 & 161.0 & 48.2 & 79.1 & 214.3 & 65.9 & 92.6 & 255.1 &  &  & \\
\bottomrule
\end{tabular}
}
\end{table*}

==> cvpr2023-author_kit-v1_1-1/tables/ablation.tex <==

\begin{table}[tb!]
\centering
\caption{\textbf{Evaluating TeachCLIP in varied setups}. For the ease of reference, performance of specific teacher models is also included. Dataset: MSRVTT-1k.}
\label{table:ablation}
\renewcommand{\arraystretch}{1.1} % Default value: 1
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lrrrr@{}}
\hline
\textbf{Model} & \textbf{R1} & \textbf{R5} & \textbf{R10} & \textbf{SumR} \\ \hline

\multicolumn{5}{@{}l}{\textit{Teacher:}} \\
X-CLIP \cite{xclip} & 45.3 & 73.7 & 81.8 & 200.8 \\
TS2-Net \cite{ts2net} & 46.7 & 72.6 & 81.2 & 200.5 \\
X-Pool \cite{xpool} & 46.0 & 72.8 & 82.7 & 201.5 \\
X-CLIP (ViT-B/16) & 49.1 & 76.1 & 84.4 & 209.6 \\ [2pt]
\multicolumn{5}{@{}l}{\textit{Student:}} \\
0: CLIP4Clip \cite{clip4clip} & 42.8 & 71.6 & 81.1 & 195.5 \\
1: CLIP4Clip(ViT-B/16) & 45.4 & 73.5 & 82.3 & 201.2 \\
2: \#0 + AFA & 44.0 & 71.2 & 81.1 & 196.3 \\ [2pt]
\multicolumn{5}{@{}l}{\textit{Student, taught by X-CLIP:}} \\
3: \#0 + CgT & 44.2 & 71.7 & 80.6 & 196.5 \\
4: \#2 + CgT & 44.4 & 71.0 & 82.6 & 198.0 \\
5: \#2 + CgT (Huber as $\ell_{CgT}$) & 44.7 & 71.1 & 82.0 & 197.8 \\
6: \#2 + FgT & 44.1 & 71.2 & 82.0 & 197.3 \\
7: \#2 + MgT & 45.2 & 72.3 & 82.3 & 199.8 \\
8: \#2 + MgT(CE as $\ell_{FgT}$) & 45.2 & 72.3 & 82.3 & 199.8 \\
9: \#2 + MgT(Pearson as $\ell_{FgT}$) & 45.4 & 73.0 & 81.3 & 199.7 \\
10: \#2 + MgT(Huber as $\ell_{FgT}$) & 45.6 & 71.9 & 81.8 & 199.3 \\ [2pt]

\multicolumn{5}{@{}l}{\textit{Student, taught by others:}} \\
11: \#7, by TS2-Net & 45.6 & 72.1 & 81.7 & 199.4 \\
12: \#7, by X-Pool & 44.0 & 73.5 & 82.6 & 200.1 \\
13: \#7, by X-CLIP \& TS2-Net  & 44.8 & 73.5 & 82.9 & 201.2 \\ 
14: \#7, by X-CLIP(ViT-B/16) & 48.1 & 75.4 & 83.5 & 207.0 \\
\hline
\end{tabular}
}
\end{table}


==> cvpr2023-author_kit-v1_1-1/tables/all_dataset.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{table*}[ht!]
\centering
\caption{\textbf{T2VR Performance of different methods on multiple datasets}. Note that we replicate existing methods with their author-provided source code where applicable, so the numbers might differ (slightly) from their original papers.
%MSRVTT-1k, MSRVTT-3k, VATEX, MSVD and ActivityNet.} Baseline models marked with * are our replication using their author-provided source code.
}
\label{table:alldatasets}
% \setlength{\tabcolsep}{3pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.1} % Default value: 1
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lrrrrrrrrrrrrrrrrrrrrrr@{}}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\makecell[c]{FLOPs\\(k)$\downarrow$}} & \multirow{2}{*}{\makecell[c]{Store\\(KB)$\downarrow$}} & \multicolumn{3}{c}{\textbf{MSRVTT-1k}} &\multicolumn{3}{c}{\textbf{MSRVTT-3k}} & \multicolumn{3}{c}{\textbf{MSVD}} & \multicolumn{3}{c}{\textbf{VATEX}} & \multicolumn{3}{c}{\textbf{ActNetCap}} \\ 
\cmidrule(r){4-6} \cmidrule(r){7-9} \cmidrule(r){10-12} \cmidrule(r){13-15} \cmidrule(r){16-18}
 & & & R1 & R5 & SumR & R1 & R5 & SumR & R1 & R5 & SumR & R1 & R5 & SumR & R1 & R5 & SumR \\ \hline
\multicolumn{17}{@{}l}{\textit{Feature re-learning w/o CLIP feature}:}\\
W2VV++, MM19 \cite{w2vv++} & 2.0 & 8 & 18.9 & 45.3 & 121.7 & 11.1 & 29.6 & 81.2 & 22.4 & 51.6 & 138.8 & - & - & - & - & -  & - \\
DualE, PAMI21 \cite{dualencoding} & 2.0 & 8 & 21.1 & 48.7 & 130.0 & 11.6 & 30.3  & 83.2 & - & - & - & 36.8 & 73.6  & 194.1 & -  & - & - \\
CE, BMVC19 \cite{ce} & 6.1 & 27 & 20.9 & 48.8  & 132.1 & 10.0 & 29.0  & 80.2 & 19.8 & 49.0 & 132.6 & - & -  & - & 17.7 & 46.6 &  - \\
SEA, TMM21 \cite{sea} &  10.2 & 40 & 23.8 & 50.3  & 137.9 & 13.1 & 33.4  & 91.5 & 24.6 & 55.0  & 147.5 & - & -  & - & - & -  & - \\
MMT, ECCV20 \cite{mmt} & 3.6 & 14 & 24.6 & 54.0  & 145.7 & - & -  & - & - & - & - & - & -  & - & 22.7 & 54.2  & - \\
TeachText, ICCV21 \cite{teachtext} & 0.8 & 3 & 29.6 & 61.6  & 165.4 & 15.0 & 38.5  & 105.2 & 25.4 & 56.9  & 153.6 & 53.2 & 87.4  & 233.9  & 23.5 & 57.2  & - \\ [3pt]
\multicolumn{17}{@{}l}{\textit{Feature re-learning with CLIP feature}:}\\
SEA  & 10.2 & 40 & 37.2 & 67.1  & 182.6 & 19.9 & 44.3  & 120.7 & 34.5 & 68.8  & 183.8 & 52.4 & 90.2  & 238.5 & - & -  & - \\
W2VV++  & 2.0 & 8 & 39.4 & 68.1  & 185.6 & 23.0 & 49.0 & 132.7 & 37.8 & 71.0 &  190.4 & 55.8 & 91.2 & 243.0 & - & -  & - \\
MMT  & 3.6 & 14 & 39.5 & 68.3  & 186.1 & 24.9 & 50.5 &  137.4 & 40.6 & 72.0 & 194.3 & 54.4 & 89.2  & 238.6 & - & - & - \\
LAFF, ECCV22 \cite{laff} & 4.1 & 16 & 45.8 & 71.5  & 199.3 & 29.1 & 54.9  & 149.8 & 45.4 & 70.6 & 200.6 & 59.1 & 91.7 & 247.1 & - & - & -  \\  [3pt]
\multicolumn{17}{@{}l}{\textit{CLIP-based end-to-end}:}\\
CenterCLIP, SIGIR22\cite{centerclip} & 1.5$\sim$7.7 & 6$\sim$30 &  44.2 & 71.6 & 197.9 & - & - & -  & 47.3 & 76.8  & 209.7 & - & - & - & 43.9 & \textbf{74.6}  & \textbf{204.3} \\
CLIP4Clip, Neurocom22 \cite{clip4clip} & \textbf{0.5} & \textbf{2} & 42.8 & 71.6  & 195.5 & 29.4 & 54.9 & 150.1 & 45.6 & 76.1  & 206.6 & 61.6 & 91.1  & 248.5 & 39.7 & 71.0  & 194.1 \\
TS2-Net, ECCV22 \cite{ts2net} & 6.1$\sim$32.8 & 24$\sim$128 & \textbf{46.7} & 72.6  & 200.5 & 29.9 & 56.4  & 153.6 & 44.6 & 75.8  & 204.9 & 61.1 & 91.5  & 248.6 & 37.3 & 69.9  & 190.4 \\
X-CLIP, MM22 \cite{xclip} & 220.9$\sim$2175.9 & 26$\sim$130 & 45.3 & \textbf{73.7} & 200.8 & \textbf{31.2} & \textbf{57.4} &  \textbf{156.7} & 47.2 & 77.0  & 210.1 & 62.2 & 90.9  & 248.5 & \textbf{44.4} & \textbf{74.6}  & 204.1 \\
X-Pool, CVPR22 \cite{xpool} & 275.0 & 24 & 46.0 & 72.8 &  \textbf{201.5}  & - & - & - & - & - & - & - & - & - & - & - & - \\
[3pt]
%\emph{This paper}: \\  %\hline
% \multicolumn{17}{l}{\textit{TS2-Net as teacher}} \\ 
TeachCLIP(X-CLIP) & \textbf{0.5} & \textbf{2} & 45.2 & 72.3 & 199.8 & 30.4 & 56.3 & 153.4 & \textbf{47.4} & \textbf{77.3} &  \textbf{210.2} & \textbf{63.6} & \textbf{91.9} &  \textbf{251.6} & 42.2 & 72.7 & 200.1  \\ 
\bottomrule
\end{tabular}
}
\end{table*}

% 暂时不需要的结果
% TeachCLIP(X-Pool) & \textbf{1} & \textbf{4} & 44.7  & 73.0  & 82.1 & 199.8 & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
% % \multicolumn{17}{l}{\textit{X-CLIP as teacher}} \\
% TeachCLIP(TS2-Net) & \textbf{1} & \textbf{4} & 45.6 & 72.1 & 81.7 & 199.4  & 30.6 & 56.3 & 66.5 & 153.4 & 62.7 & 91.8 & 96.2 & 250.7 & 47.0 & 77.2 & 85.6 & 209.8 & 41.5 & 72.5 & 84.4 & 198.4  \\ %\hline




%原始结果
% CLIP4Clip \cite{clip4clip} & - & - & - & - & - & - & - & - & 45.2 & 75.5 & 84.3 & 205.0 & 40.5 & 72.4 & - & - \\
% X-CLIP \cite{xclip} & - & - & - & - & - & - & - & - & 47.1 & 77.8 & - & - & 44.3 & 74.1 & - & - \\
%TS2-Net \cite{ts2net} & - & - & - & - & 59.1 & 90.0 & 95.2 & 244.3 & - & - & - & - & 41.0 & 73.6 & 84.5 & 199.1 \\

% X-Pool \cite{xpool} & - & - & - & - & - & - & - & - & 47.2 & 77.4 & 86.0 & 210.6 & - & - & - & - \\

% CLIP2Video \cite{clip2video} & - & - & - & - & 57.3 & 90.0 & 95.5 & 242.8 & 47.0 & 76.8 & \textbf{85.9} & 209.7 & - & - & - & - \\
% CLIP2Video\cite{clip2video} & 2 & 8 & 45.6 & 72.6 & 199.9 & - & - & - & 57.3 & 90.0  & 242.8 & 47.0 & 76.8 & 209.7 & - & - & -  \\




% \begin{table*}[ht!]
% \centering
% \caption{\textbf{T2VR Performance of different methods on multiple datasets}. Note that we replicate existing methods with their author-provided source code where applicable, so the numbers might differ (slightly) from their original papers.
% %MSRVTT-1k, MSRVTT-3k, VATEX, MSVD and ActivityNet.} Baseline models marked with * are our replication using their author-provided source code.
% }
% \label{table:alldatasets}
% % \setlength{\tabcolsep}{3pt} % Default value: 6pt
% \renewcommand{\arraystretch}{1.1} % Default value: 1
% \resizebox{\linewidth}{!}{
% \begin{tabular}{@{}lrrrrrrrrrrrrrrrrrrrrrr@{}}
% \toprule
% \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\makecell[c]{FLOPs\\(k)$\downarrow$}} & \multirow{2}{*}{\makecell[c]{Store\\(KB)$\downarrow$}} & \multicolumn{3}{c}{\textbf{MSRVTT-1k}} &\multicolumn{3}{c}{\textbf{MSRVTT-3k}} & \multicolumn{3}{c}{\textbf{VATEX}} & \multicolumn{3}{c}{\textbf{MSVD}} & \multicolumn{3}{c}{\textbf{ActNetCap}} \\ 
% \cmidrule(r){4-6} \cmidrule(r){7-9} \cmidrule(r){10-12} \cmidrule(r){13-15} \cmidrule(r){16-18}
%  & & & R1 & R5 & SumR & R1 & R5 & SumR & R1 & R5 & SumR & R1 & R5 & SumR & R1 & R5 & SumR \\ \hline
% \multicolumn{17}{@{}l}{\textit{Feature re-learning w/o CLIP feature}:}\\
% W2VV++, MM19 \cite{w2vv++} & 4 & 16 & 18.9 & 45.3 & 121.7 & 11.1 & 29.6 & 81.2 & - & - & - & 22.4 & 51.6 & 138.8 & - & -  & - \\
%  DualE, PAMI21 \cite{dualencoding} & 4 & 16 & 21.1 & 48.7 & 130.0 & 11.6 & 30.3  & 83.2 & 36.8 & 73.6  & 194.1 & - & - & - & -  & - & - \\
%  CE, BMVC19 \cite{ce} & & & 20.9 & 48.8  & 132.1 & 10.0 & 29.0  & 80.2 & - & -  & - & 19.8 & 49.0  & 132.6 & 17.7 & 46.6 &  - \\
%  SEA, TMM21 \cite{sea} &  20 & 80 & 23.8 & 50.3  & 137.9 & 13.1 & 33.4  & 91.5 & - & -  & - & 24.6 & 55.0  & 147.5 & - & -  & - \\
%  MMT, ECCV20 \cite{mmt} & & & 24.6 & 54.0  & 145.7 & - & -  & - & - & - & - & - & -  & - & 22.7 & 54.2  & - \\
% TeachText, ICCV21 \cite{teachtext} & 1.5 & 6 & 29.6 & 61.6  & 165.4 & 15.0 & 38.5  & 105.2 & 53.2 & 87.4  & 233.9 & 25.4 & 56.9  & 153.6 & 23.5 & 57.2  & - \\ [3pt]
% \multicolumn{17}{@{}l}{\textit{Feature re-learning with CLIP feature}:}\\
% SEA  &  20 & 80 & 37.2 & 67.1  & 182.6 & 19.9 & 44.3  & 120.7 & 52.4 & 90.2  & 238.5 & 34.5 & 68.8  & 183.8 & - & -  & - \\
% W2VV++  & 4 & 16 & 39.4 & 68.1  & 185.6 & 23.0 & 49.0 & 132.7 & 55.8 & 91.2 & 243.0 & 37.8 & 71.0 &  190.4 & - & -  & - \\
% MMT  & & & 39.5 & 68.3  & 186.1 & 24.9 & 50.5 &  137.4 & 54.4 & 89.2  & 238.6 & 40.6 & 72.0 & 194.3 & - & - & - \\
% LAFF, ECCV22 \cite{laff} & 8 & 32 & 45.8 & 71.5  & 199.3 & 29.1 & 54.9  & 149.8 & 59.1 & 91.7 & 247.1 & 45.4 & 70.6 & 200.6 & - & - & -  \\
% \multicolumn{17}{@{}l}{\textit{CLIP-based end-to-end}:}\\
% CenterCLIP, SIGIR22\cite{centerclip} & 3 & 8 &  44.2 & 71.6 & 197.9 & - & - & -  & - & - & - & 47.3 & 76.8  & 209.7 & 43.9 & \textbf{74.6}  & \textbf{204.3} \\
% CLIP4Clip, Neurocom22 \cite{clip4clip} & \textbf{1} & \textbf{4} & 42.8 & 71.6  & 195.5 & 29.4 & 54.9 & 150.1 & 61.6 & 91.1  & 248.5 & 45.6 & 76.1  & 206.6 & 39.7 & 71.0  & 194.1 \\
%  TS2-Net, ECCV22 \cite{ts2net} & 12 & 26 & \textbf{46.7} & 72.6  & 200.5 & 29.9 & 56.4  & 153.6 & 61.1 & 91.5  & 248.6 & 44.6 & 75.8  & 204.9 & 37.3 & 69.9  & 190.4 \\
% X-CLIP, MM22 \cite{xclip} & 384 & 88 & 45.3 & \textbf{73.7} & 200.8 & \textbf{31.2} & \textbf{57.4} &  \textbf{156.7} & 62.2 & 90.9  & 248.5 & 47.2 & 77.0  & 210.1 & \textbf{44.4} & \textbf{74.6}  & 204.1 \\
% X-Pool, CVPR22 \cite{xpool} & 512 & 26 & 46.0 & 72.8 &  \textbf{201.5}  & - & - & - & - & - & - & - & - & - & - & - & - \\
% [3pt]
% %\emph{This paper}: \\  %\hline
% % \multicolumn{17}{l}{\textit{TS2-Net as teacher}} \\ 
% TeachCLIP(X-CLIP) & \textbf{1} & \textbf{4} & 45.2 & 72.3 & 199.8 & 30.4 & 56.3 & 153.4 & \textbf{63.6} & \textbf{91.9} &  \textbf{251.6} & \textbf{47.4} & \textbf{77.3} &  \textbf{210.2} & 42.2 & 72.7 & 200.1  \\ 

% \bottomrule
% \end{tabular}
% }
% \end{table*}


==> cvpr2023-author_kit-v1_1-1/tables/dataset.tex <==


\begin{table}[ht!]
\centering
\caption{\textbf{Experimental data}. MSRVTT-1k is used as the primary dataset for ablation study, while all datasets are used to compare TeachCLIP with existing methods.}
\label{tab:datasets}
% \renewcommand{\arraystretch}{1.1} % Default value: 1
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{2}{c}{\textbf{Training set}} & \multicolumn{2}{c}{\textbf{Validation set}} & \multicolumn{2}{c}{\textbf{Test set}} \\ \cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7}
 & \#videos & \#texts & \#videos & \#texts & \#videos & \#texts \\ \hline
MSRVTT-1k \cite{msrvtt-1ka} & 9,000 & 180,000 & n.a. & n.a. & 1,000 & 1,000 \\
MSRVTT-3k \cite{msrvtt} & 6,513 & 130,260 & 497 & 9,940 & 2,990 & 59,800 \\
MSVD \cite{msvd} & 1,200 & 48,774 & 100 & 4,290 & 670 & 27,763 \\
VATEX \cite{vatex} & 25,991 & 259,910 & 1,500 & 15,000 & 1,500 & 15,000 \\
ActNetCap \cite{activitynet} & 10,009 & 10,009 & n.a. & n.a. & 4,917 & 4,917 \\
\bottomrule
\end{tabular}
}
\end{table}


==> cvpr2023-author_kit-v1_1-1/tables/msrvtt1ka.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[]
% \caption{Retrieval performance comparison to SOTAs on the MSRVTT-1kA dataset.}
% \label{table:msrvtt-1ka}
% \setlength{\tabcolsep}{3pt} % Default value: 6pt
% \renewcommand{\arraystretch}{1} % Default value: 1
% \begin{tabular}{lcccccccccc}
% \toprule
%  \multirow{2}{*}{Model} & \multicolumn{4}{c}{Text-to-Video Retrieval} & \multicolumn{4}{c}{Video-to-Text Retrieval} & \multirow{2}{*}{FLOPs(k)$\downarrow$} & \multirow{2}{*}{Stor.(KB)$\downarrow$} \\ \cline{2-9}
%  & R@1$\uparrow$ & R@5$\uparrow$ & R@10$\uparrow$ & Mean$\uparrow$ & R@1$\uparrow$ & R@5$\uparrow$ & R@10$\uparrow$ & Mean$\uparrow$ &  &  \\ \hline
% TeachText\cite{teachtext} & 29.6 & 61.6 & 74.2 & 55.1 & 32.1 & 62.7 & 75.0 & 56.6 & 1.5 & 6 \\
% SEA\cite{sea} & 37.2 & 67.1 & 78.3 & 60.9 & - & - & - & - & 4 & 16 \\
% W2VV++\cite{w2vv++} & 39.4 & 68.1 & 78.1 & 61.9 & - & - & - & - & 4 & 16 \\
% CLIP4Clip\cite{clip4clip} & 42.8 & 71.6 & 81.1 & 65.2 & 41.4 & 70.6 & 80.5 & 64.2 & 1 & 4 \\
% BridgeFormer\cite{bridgeformer} & 44.9 & 71.9 & 80.3 & 65.7 & - & - & - & - & 1 & 4 \\
% CLIP2Video\cite{clip2video} & 44.9 & 72.2 & 81.3 & 66.1 & 44.4 & 72.3 & 82.2 & 66.3 & 2 & 8 \\
% LAFF\cite{laff} & 45.8 & 71.5 & 82.0 & 66.4 & - & - & - & - & 4 & 16 \\
% TS2-Net\cite{ts2net} & 46.7 & 72.6 & 81.2 & 66.8 & 43.6 & 71.1 & 82.7 & 65.8 & 12 & 26 \\
% X-CLIP\cite{xclip} & 45.3 & 73.7 & 81.9 & 67.0 & 44.9 & 73.4 & 81.9 & 66.7 & 384 & 88 \\
% X-Pool\cite{xpool} & 46.9 & 72.8 & 82.2 & 67.3 & 44.4 & 73.3 & 84.0 & 67.2 & 512 & 26 \\ \hline
% \multicolumn{11}{l}{\textit{X-CLIP as teacher, CLIP4Clip as student}} \\
% TeachCLIP-Coarse & $44.2_{\uparrow1.4}$ & $71.7_{\uparrow0.1}$ & $80.6_{\downarrow0.5}$ & $65.5_{\uparrow0.3}$ & $42.4_{\uparrow1.0}$ & $70.3_{\downarrow0.3}$ & $80.6_{\downarrow0.1}$ & $64.4_{\uparrow0.2}$ & 1 & 4 \\
% TeachCLIP-Fine & $45.2_{\uparrow2.4}$ & $72.3_{\uparrow0.7}$ & $82.3_{\uparrow1.2}$ & $66.6_{\uparrow1.4}$ & $43.6_{\uparrow2.2}$ & $71.3_{\uparrow0.7}$ & $81.6_{\uparrow1.1}$ & $65.5_{\uparrow1.3}$ & 1 & 4 \\ \hline
% \multicolumn{11}{l}{\textit{TS2-Net as teacher, CLIP4Clip as student}} \\
% TeachCLIP-Coarse & $44.0_{\uparrow1.2}$ & $71.3_{\downarrow0.3}$ & $81.1_{\uparrow0.0}$ & $65.5_{\uparrow0.3}$ & $41.2_{\downarrow0.2}$ & $69.5_{\downarrow1.1}$ & $80.5_{\uparrow0.0}$ & $63.7_{\downarrow0.5}$ & 1 & 4 \\
% TeachCLIP-Fine & $45.6_{\uparrow2.8}$ & $72.1_{\uparrow0.5}$ & $81.7_{\uparrow0.6}$ & $66.5_{\uparrow1.3}$ & $43.0_{\uparrow1.6}$ & $71.4_{\uparrow0.8}$ & $81.4_{\uparrow0.9}$ & $65.3_{\uparrow1.1}$ & 1 & 4 \\ \hline
% \end{tabular}
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[ht!]
\caption{\textbf{T2VR performance on MSRVTT-1k}. Baseline models marked with * are our replication using their author-provided source code. Baselines sorted in ascending order by SumR, \ie. sum of R1, R5 and R10.}
\label{table:msrvtt-1ka}
%\setlength{\tabcolsep}{2pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.1} % Default value: 1
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
\textbf{Model} &   R1$\uparrow$ & R5$\uparrow$ & R10$\uparrow$ & SumR$\uparrow$ & \makecell[c]{FLOPs\\(k)$\downarrow$} & \makecell[c]{Store\\(KB)$\downarrow$} \\ \hline
\multicolumn{7}{@{}l}{\textit{Feature re-learning w/o CLIP feature}:} \\
W2VV++ \cite{w2vv++} & 18.9 & 45.3 & 57.5 & 121.7 & 4 & 16 \\
DualE \cite{dualencoding} & 21.1 & 48.7 & 60.2 & 130.0 & 4 & 16 \\
CE \cite{ce} & 20.9 & 48.8 & 62.4 & 132.1 &  &  \\
SEA \cite{sea} & 23.8 & 50.3 & 63.8 & 137.9 & 20 & 80 \\
MMT \cite{mmt} & 24.6 & 54.0 & 67.1 & 145.7 &  & \\
TeachText \cite{teachtext} & 29.6 & 61.6 & 74.2 & 165.4 & 1.5 & 6 \\
\multicolumn{7}{@{}l}{\textit{Feature re-learning with CLIP feature}:}\\
SEA \cite{sea} & 37.2 & 67.1 & 78.3 & 182.6 & 20 & 80 \\
W2VV++ \cite{w2vv++} & 39.4 & 68.1 & 78.1 & 185.6 & 4 & 16 \\
MMT \cite{mmt} & 39.5 & 68.3 & 78.3 & 186.1 &  & \\
LAFF \cite{laff} & 45.8 & 71.5 & 82.0 & 199.3 & 8 & 32 \\
\multicolumn{7}{@{}l}{\textit{CLIP-based end-to-end}:}\\
CLIP4Clip* \cite{clip4clip} & 42.8 & 71.6 & 81.1 & 195.5 & \textbf{1} & \textbf{4} \\
CenterCLIP \cite{centerclip} & 44.2 & 71.6 & 82.1 & 197.9 & 3 & 8 \\
TS2-Net* \cite{ts2net} & \textbf{46.7} & 72.6 & 81.2 & 200.5 & 12 & 26 \\ 
X-CLIP* \cite{xclip} & 45.3 & \textbf{73.7} & 81.8 & 200.8 & 384 & 88 \\
X-Pool* \cite{xpool} & 46.0 & 72.8 & \textbf{82.7} & \textbf{201.5} & 512 & 26 \\
[3pt] %\hline
\emph{This paper}: \\  %\hline
%\multicolumn{7}{l}{\textit{X-CLIP as teacher}} \\
%\multicolumn{7}{l}{\textit{TS2-Net as teacher}} \\
TeachCLIP(TS2-Net) & 45.6 & 72.1 & 81.7 & 199.4 & \textbf{1} & \textbf{4} \\ 
TeachCLIP(X-CLIP) & 45.2 & 72.3 & 82.3 & 199.8 & \textbf{1} & \textbf{4} \\
TeachCLIP(X-Pool) & 44.7  & 73.0  & 82.1 & 199.8 & \textbf{1} & \textbf{4} \\ %\hline
\bottomrule
\end{tabular}
}
\end{table}


% 原始的结果
% CLIP4Clip \cite{clip4clip} & 44.5 & 71.4 & 81.6 & 197.5 & 1 & 4 \\
% X-CLIP \cite{xclip} & 46.1 & 73.0 & 83.1 & 202.2 & 384 & 88 \\
%TS2-Net \cite{ts2net} & 47.0 & 74.5 & 83.8 & 205.3 & 12 & 26 \\

% X-Pool \cite{xpool} & \textbf{46.9} & 72.8 & 82.2 & \textbf{201.9} & 512 & 26 \\

% CLIP2Video \cite{clip2video} & 45.6 & 72.6 & 81.7 & 199.9 & 2 & 8 \\
% BridgeFormer \cite{bridgeformer} & 44.9 & 71.9 & 80.3 & 197.1 & 1 & 4 \\

==> cvpr2023-author_kit-v1_1-1/tables/otherdataset.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{table*}[ht!]
\centering
\caption{\textbf{T2VR performance on MSRVTT-3k, VATEX, MSVD and ActivityNet.}}
\label{table:others}
% \setlength{\tabcolsep}{3pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.1} % Default value: 1
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lccrrrrrrrrrrrrrrrrrrrr@{}}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{FLOPs} & \multirow{2}{*}{Store} & \multicolumn{4}{c}{MSRVTT-1k} &\multicolumn{4}{c}{MSRVTT-3k} & \multicolumn{4}{c}{VATEX} & \multicolumn{4}{c}{MSVD} & \multicolumn{4}{c}{ActivityNet} \\ 
\cmidrule(r){4-7} \cmidrule(r){8-11} \cmidrule(r){12-15} \cmidrule(r){16-19} \cmidrule(r){20-23}
 & & & R1 & R5 & R10 & SumR & R1 & R5 & R10 & SumR & R1 & R5 & R10 & SumR & R1 & R5 & R10 & SumR & R1 & R5 & R10 & SumR \\ \hline
\multicolumn{17}{@{}l}{\textit{Feature re-learning w/o CLIP feature}:}\\
W2VV++ \cite{w2vv++} & 4 & 16 & 18.9 & 45.3 & 57.5 & 121.7 & 11.1 & 29.6 & 40.5 & 81.2 & - & - & - & - & 22.4 & 51.6 & 64.8 & 138.8 & - & - & - & - \\
 DualE \cite{dualencoding} & 4 & 16 & 21.1 & 48.7 & 60.2 & 130.0 & 11.6 & 30.3 & 41.3 & 83.2 & 36.8 & 73.6 & 83.7 & 194.1 & - & - & - & - & - & - & - & - \\
 CE \cite{ce} & & & 20.9 & 48.8 & 62.4 & 132.1 & 10.0 & 29.0 & 41.2 & 80.2 & - & - & - & - & 19.8 & 49.0 & 63.8 & 132.6 & 17.7 & 46.6 & - & - \\
 SEA \cite{sea} &  20 & 80 & 23.8 & 50.3 & 63.8 & 137.9 & 13.1 & 33.4 & 45.0 & 91.5 & - & - & - & - & 24.6 & 55.0 & 67.9 & 147.5 & - & - & - & - \\
 MMT \cite{mmt} & & & 24.6 & 54.0 & 67.1 & 145.7 & - & - & - & - & - & - & - & - & - & - & - & - & 22.7 & 54.2 & - & - \\
TeachText \cite{teachtext} & 1.5 & 6 & 29.6 & 61.6 & 74.2 & 165.4 & 15.0 & 38.5 & 51.7 & 105.2 & 53.2 & 87.4 & 93.3 & 233.9 & 25.4 & 56.9 & 71.3 & 153.6 & 23.5 & 57.2 & - & - \\
\multicolumn{17}{@{}l}{\textit{Feature re-learning with CLIP feature}:}\\
SEA \cite{sea} &  20 & 80 & 37.2 & 67.1 & 78.3 & 182.6 & 19.9 & 44.3 & 56.5 & 120.7 & 52.4 & 90.2 & 95.9 & 238.5 & 34.5 & 68.8 & 80.5 & 183.8 & - & - & - & - \\
W2VV++ \cite{w2vv++} & 4 & 16 & 39.4 & 68.1 & 78.1 & 185.6 & 23.0 & 49.0 & 60.7 & 132.7 & 55.8 & 91.2 & 96.0 & 243.0 & 37.8 & 71.0 & 81.6 & 190.4 & - & - & - & - \\
MMT \cite{mmt} & & & 39.5 & 68.3 & 78.3 & 186.1 & 24.9 & 50.5 & 62.0 & 137.4 & 54.4 & 89.2 & 95.0 & 238.6 & 40.6 & 72.0 & 81.7 & 194.3 & - & - & - & - \\
LAFF \cite{laff} & 8 & 32 & 45.8 & 71.5 & 82.0 & 199.3 & 29.1 & 54.9 & 65.8 & 149.8 & 59.1 & 91.7 & \textbf{96.3} & 247.1 & 45.4 & 70.6 & 84.6 & 200.6 & - & - & - & - \\
\multicolumn{17}{@{}l}{\textit{CLIP-based end-to-end}:}\\
CenterCLIP\cite{centerclip} & 3 & 8 &  44.2 & 71.6 & 82.1 & 197.9 & - & - & - & - & - & - & - & - & 47.3 & 76.8 & 85.6 & 209.7 & 43.9 & \textbf{74.6} & \textbf{85.8} & \textbf{204.3} \\
CLIP4Clip* \cite{clip4clip} & \textbf{1} & \textbf{4} & 42.8 & 71.6 & 81.1 & 195.5 & 29.4 & 54.9 & 65.8 & 150.1 & 61.6 & 91.1 & 95.8 & 248.5 & 45.6 & 76.1 & 84.9 & 206.6 & 39.7 & 71.0 & 83.4 & 194.1 \\
 TS2-Net* \cite{ts2net} & 12 & 26 & \textbf{46.7} & 72.6 & 81.2 & 200.5 & 29.9 & 56.4 & 67.3 & 153.6 & 61.1 & 91.5 & 96.0 & 248.6 & 44.6 & 75.8 & 84.5 & 204.9 & 37.3 & 69.9 & 83.2 & 190.4 \\
X-CLIP* \cite{xclip} & 384 & 88 & 45.3 & \textbf{73.7} & 81.8 & 200.8 & \textbf{31.2} & \textbf{57.4} & \textbf{68.1} & \textbf{156.7} & 62.2 & 90.9 & 95.4 & 248.5 & 47.2 & 77.0 & \textbf{85.9} & 210.1 & \textbf{44.4} & \textbf{74.6} & 85.1 & 204.1 \\
X-Pool* \cite{xpool} & 512 & 26 & 46.0 & 72.8 & \textbf{82.7} & \textbf{201.5} & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
[3pt]
\emph{This paper}: \\  %\hline
% \multicolumn{17}{l}{\textit{X-CLIP as teacher}} \\
TeachCLIP(TS2-Net) & \textbf{1} & \textbf{4} & 45.6 & 72.1 & 81.7 & 199.4  & 30.6 & 56.3 & 66.5 & 153.4 & 62.7 & 91.8 & 96.2 & 250.7 & 47.0 & 77.2 & 85.6 & 209.8 & 41.5 & 72.5 & 84.4 & 198.4  \\ %\hline
% \multicolumn{17}{l}{\textit{TS2-Net as teacher}} \\ 
TeachCLIP(X-CLIP) & \textbf{1} & \textbf{4} & 45.2 & 72.3 & 82.3 & 199.8 & 30.4 & 56.3 & 66.7 & 153.4 & \textbf{63.6} & \textbf{91.9} & 96.1 & \textbf{251.6} & \textbf{47.4} & \textbf{77.3} & 85.5 & \textbf{210.2} & 42.2 & 72.7 & 85.4 & 200.1  \\ 
TeachCLIP(X-Pool) & \textbf{1} & \textbf{4} & 44.7  & 73.0  & 82.1 & 199.8 & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
\bottomrule
\end{tabular}
}
\end{table*}


%原始结果
% CLIP4Clip \cite{clip4clip} & - & - & - & - & - & - & - & - & 45.2 & 75.5 & 84.3 & 205.0 & 40.5 & 72.4 & - & - \\
% X-CLIP \cite{xclip} & - & - & - & - & - & - & - & - & 47.1 & 77.8 & - & - & 44.3 & 74.1 & - & - \\
%TS2-Net \cite{ts2net} & - & - & - & - & 59.1 & 90.0 & 95.2 & 244.3 & - & - & - & - & 41.0 & 73.6 & 84.5 & 199.1 \\

% X-Pool \cite{xpool} & - & - & - & - & - & - & - & - & 47.2 & 77.4 & 86.0 & 210.6 & - & - & - & - \\

% CLIP2Video \cite{clip2video} & - & - & - & - & 57.3 & 90.0 & 95.5 & 242.8 & 47.0 & 76.8 & \textbf{85.9} & 209.7 & - & - & - & - \\



==> tables/ab_afa.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table}[ht!]
% \caption{\textbf{Ablation study of AFA module on MSRVTT-1k.}}
% \label{ab_afa}
% % \setlength{\tabcolsep}{6pt} % Default value: 6pt
% \renewcommand{\arraystretch}{1} % Default value: 1
% % \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{@{}llrrrr@{}}
% \toprule
% Activation & \#Linear & R1 & R5 & R10 & SumR \\ \hline
% - & 1 & 44.9 & 72.2 & 81.9 & 199.0 \\
% ReLU & 2 & 45.2 & 72.3 & 82.3 & 199.8 \\
% Sigmoid & 2 & 44.8 & 72.9 & 82.0 & 199.7 \\
% tanh & 2 & 44.8 & 72.9 & 82.1 & 199.8 \\
% ReLU & 3 & 44.2 & 73.2 & 82.0 & 199.4 \\
% \bottomrule
% \end{tabular}
% }
% \end{table}

\begin{table}[ht!]
\caption{\textbf{Influence of the number of FC layers in AFA on the text-to-video retrieval performance}. Dataset: MSRVTT-1k. Teacher network: X-CLIP.} 
\label{ab_afa}
\setlength{\tabcolsep}{16pt} % Default value: 6pt
\renewcommand{\arraystretch}{1} % Default value: 1
% \centering
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lrrrr@{}}
\toprule
\textbf{\#FC layers} & \textbf{R1} & \textbf{R5} & \textbf{R10} & \textbf{SumR} \\ \hline
1 & 44.9 & 72.2 & 81.9 & 199.0 \\
2 (used in the paper) & 45.2 & 72.3 & 82.3 & 199.8 \\
3 & 44.2 & 73.2 & 82.0 & 199.4 \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/ab_fineloss.tex <==


\begin{table}[ht!]
\caption{\textbf{Ablation study of $\ell_{FgT}$.} Teacher:X-CLIP,Studnet:CLIP4Clip-AFA, $\ell_{CgT}$: Pearson Distance}
\label{ab_loss}
\renewcommand{\arraystretch}{1}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}llllllr@{}}
\hline
 & 1k & \multicolumn{1}{r}{3k} & \multicolumn{1}{r}{VA.} & \multicolumn{1}{r}{MS.} & \multicolumn{1}{r}{Ac.} & Mean \\ \hline
Huber & 199.3 & 154.6 & 250.5 & 209.9 & 197.8 & 202.4 \\
Cross Entropy & 199.8 & 153.4 & 251.5 & 210.2 & 200.1 & 203.0 \\
Pearson & 199.7 & 152.1 & 249.4 & 209.2 & 198.3 & 201.7 \\ \hline
\end{tabular}
}
\end{table}



% \setlength{\tabcolsep}{3pt} % Default value: 6pt
% Default value: 1

==> tables/ab_loss.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[ht!]
\caption{\textbf{Ablation study of $\ell_{ct}$.}}
\label{ab_loss}
% \setlength{\tabcolsep}{3pt} % Default value: 6pt
\renewcommand{\arraystretch}{1} % Default value: 1
% \centering
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
Distance Metric & 1k & 3k & VA. & MS. & Ac. & Mean \\ \hline
Huber & 197.8 & 150.0 & 247.5 & 205.0 & 180.2 & 196.1 \\
Cross Entropy & 198.2 & 150.6 & 249.3 & 207.0 & 196.5 & 200.3 \\
Pearson & 196.5 & 151.8 & 250.0 & 208.4 & 197.3 & 200.8 \\ \bottomrule
\end{tabular}
}
\end{table}


==> tables/ab_multi.tex <==

\begin{table}[ht!]
\caption{\textbf{Ablation study of multi-teacher teaching.}}
\label{ab_multi}
% \setlength{\tabcolsep}{1pt} % Default value: 6pt
\renewcommand{\arraystretch}{1} % Default value: 1
% \centering
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lrrrrrr@{}}
\hline
 & 1k & 3k & VA. & MS. & Ac. & Mean \\ \hline
TeachCLIP(TS2Net) & \multicolumn{1}{l}{199.4} & 153.4 & 250.7 & 209.8 & \multicolumn{1}{l}{198.4} & 202.3 \\
TeachCLIP(XCLIP) & \multicolumn{1}{l}{199.8} & 153.4 & 251.5 & 210.2 & \multicolumn{1}{l}{200.1} & 203.0 \\
TeachCLIP(TS2Net,XCLIP) & 201.2 & 154.9 & 251.5 & 210.6 & 201.4 & 203.9 \\ \hline
\end{tabular}
}
\end{table}

% CLIP4Clip & 195.5 & 150.1 & \multicolumn{1}{r}{248.5} & \multicolumn{1}{r}{206.6} & 196.9 & 199.52 \\
% TS2Net & 200.5 & 153.6 & \multicolumn{1}{r}{248.6} & \multicolumn{1}{r}{204.9} & 190.4 & 199.6 \\
% X-CLIP & 200.8 & 156.7 & \multicolumn{1}{r}{248.5} & \multicolumn{1}{r}{209.0} & 204.1 & 203.82 \\

==> tables/ab_student.tex <==
\begin{table}[ht!]
\caption{\textbf{Ablation study of student network.} We use 1k, 3k, VA., MS., and Ac. to respectively represent the abbreviations of MSRVTT-1k, MSRVTT-3k, VATEX, MSVD, and ActivityNet. The evaluation metric is SumR, and Mean is the average of SumR across multiple datasets.}
\label{ab_student}
% \setlength{\tabcolsep}{1pt} % Default value: 6pt
\renewcommand{\arraystretch}{1} % Default value: 1
% \centering
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lrrrrrrrr@{}}
\toprule
Student network & $l_{ct}$ & $l_{ft}$ & 1k & 3k & VA. & MS. & Ac. & Mean \\ \hline
\multirow{2}{*}{CLIP4Clip} & \ding{55} & n.a. & 195.5 & 150.1 & 248.5 & 206.6 & 194.1 & 199.0 \\
 & \checkmark & n.a. & 196.5 & 151.8 & 250.0 & 208.4 & 197.3 & 200.8 \\ \hline
\multirow{3}{*}{CLIP4Clip-AFA} & \ding{55} & \ding{55} & 196.3 & 152.1 & 249.4 & 208.2 & 194.8 & 200.2 \\
 & \checkmark & \ding{55} & 198.0 & 152.7 & 250.3 & 209.8 & 198.5 & 201.9 \\
 & \checkmark & \checkmark & 199.8 & 153.4 & 251.5 & 210.2 & 200.1 & 203.0 \\ \bottomrule
\end{tabular}
}
\end{table}
% 这里我们使用1k，3k, VA., MS., Ac. 分别代表MSRVTT-1k,MSRVTT-3k,VATEX,MSVD 和ActivityNet的缩写。 衡量指标是SumR，Mean 是多个数据集SumR的平均值。

==> tables/ab_temp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{\textbf{Ablation study of temperature on MSRVTT-1k.}}
\label{ab_temp}
% \setlength{\tabcolsep}{6pt} % Default value: 6pt
\renewcommand{\arraystretch}{1} % Default value: 1
% \centering
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lrrrr@{}}
\toprule
Temperature & R1 & R5 & R10 & SumR \\ \hline
0.5 & 44.6 & 71.6 & 80.0 & 196.2 \\
1.0 & 44.2 & 71.7 & 80.6 & 196.5 \\
2.0 & 43.3 & 71.0 & 81.3 & 195.6 \\
5.0 & 43.5 & 71.3 & 80.8 & 195.6 \\ \bottomrule
\end{tabular}
}
\end{table}

==> tables/ab_vit16.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table}[ht!]
% \caption{\textbf{CLIP(ViT-B/16) on MSRVTT-1k.}}
% \label{ab_vit16}
% \renewcommand{\arraystretch}{1} % Default value: 1
% % \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{@{}lrrrr@{}}
% \toprule
% Model & R1 & R5 & R10 & SumR \\ \hline
% CLIP4Clip & 45.4 & 73.5 & 82.3 & 201.2 \\
% X-CLIP & 49.1 & 76.1 & 84.4 & 209.6   \\
% TeachCLIP(X-CLIP) & 48.1 & 75.4 & 83.5 & 207.0 \\ 
% \bottomrule
% \end{tabular}
% }
% \end{table}

 
 
 

 % Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[ht!]
\caption{\textbf{Ablation study of visual encoder on multiple datasets.}}
\label{ab_vit16}
\renewcommand{\arraystretch}{1} % Default value: 1
% \centering
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lrrrrrrrrrrrrrrr@{}}
\toprule
\multirow{2}{*}{\textbf{model}} & \multicolumn{3}{c}{\textbf{MSRVTT-1k}} & \multicolumn{3}{c}{\textbf{MSRVTT-3k}} & \multicolumn{3}{c}{\textbf{MSVD}} & \multicolumn{3}{c}{\textbf{VATEX}} & \multicolumn{3}{c}{\textbf{ActNetCap}} \\
\cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){8-10} \cmidrule(r){11-13} \cmidrule(r){14-16} 
 & R1 & R5 & SumR & R1 & R5 & SumR & R1 & R5 & SumR & R1 & R5 & SumR & R1 & R5 & SumR \\ \hline
 \multicolumn{16}{@{}l}{\textit{ViT-B/32 as visual encoder}:}\\
 CenterCLIP \cite{centerclip} &  44.2 & 71.6 & 197.9 & - & - & -  & 47.3 & 76.8  & 209.7 & - & - & - & 43.9 & 74.6 & 204.3 \\
 CLIP4Clip \cite{clip4clip} & 42.8 & 71.6 & 195.5 & 29.4 & 54.9 & 150.1 & 45.6 & 76.1 & 206.6 & 61.6 & 91.1 & 248.5 & 39.7 & 71.0 & 194.1 \\
X-CLIP \cite{xclip} & 45.3 & 73.7 & 200.8 & 31.2 & 57.4 & 156.7 & 47.2 & 77.0 & 210.1 & 62.2 & 90.9 & 248.5 & 44.4 & 74.6 & 204.1 \\
TeachCLIP(X-CLIP) & 44.0 & 73.5 & 200.1 & 30.4 & 56.3 & 153.4 & 47.4 & 77.3 & 210.2 & 63.6 & 91.9 & 251.6 & 42.2 & 72.7 & 200.1 \\
[3pt]
\multicolumn{16}{@{}l}{\textit{ViT-B/16 as visual encoder}:}\\
CenterCLIP & 48.4 & 73.8 & 204.2 & - & - & - & 50.6 & 80.3 & 219.3 & - & - & - & 46.2 & 77.0 & 210.8 \\
CLIP4Clip & 45.4 & 73.5 & 201.2 & 31.3 & 56.9 & 155.6 & 47.1 & 77.9 & 211.4 & 64.7 & 92.1 & 253.3 & 40.3 & 71.6 & 195.1 \\
X-CLIP & 49.1 & 76.1 & 209.6 & 33.4 & 59.3 & 162.0 & 48.2 & 78.7 & 213.8 & 65.8 & 92.5 & 254.7 & 44.8 & 74.2 & 204.5 \\
TeachCLIP(X-CLIP) & 48.1 & 75.4 & 207.0 & 32.8 & 58.9 & 161.0 & 48.2 & 79.1 & 214.3 & 65.9 & 92.6 & 255.1 &  &  & \\
\bottomrule
\end{tabular}
}
\end{table*}

==> tables/msrvtt1ka.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[]
% \caption{Retrieval performance comparison to SOTAs on the MSRVTT-1kA dataset.}
% \label{table:msrvtt-1ka}
% \setlength{\tabcolsep}{3pt} % Default value: 6pt
% \renewcommand{\arraystretch}{1} % Default value: 1
% \begin{tabular}{lcccccccccc}
% \toprule
%  \multirow{2}{*}{Model} & \multicolumn{4}{c}{Text-to-Video Retrieval} & \multicolumn{4}{c}{Video-to-Text Retrieval} & \multirow{2}{*}{FLOPs(k)$\downarrow$} & \multirow{2}{*}{Stor.(KB)$\downarrow$} \\ \cline{2-9}
%  & R@1$\uparrow$ & R@5$\uparrow$ & R@10$\uparrow$ & Mean$\uparrow$ & R@1$\uparrow$ & R@5$\uparrow$ & R@10$\uparrow$ & Mean$\uparrow$ &  &  \\ \hline
% TeachText\cite{teachtext} & 29.6 & 61.6 & 74.2 & 55.1 & 32.1 & 62.7 & 75.0 & 56.6 & 1.5 & 6 \\
% SEA\cite{sea} & 37.2 & 67.1 & 78.3 & 60.9 & - & - & - & - & 4 & 16 \\
% W2VV++\cite{w2vv++} & 39.4 & 68.1 & 78.1 & 61.9 & - & - & - & - & 4 & 16 \\
% CLIP4Clip\cite{clip4clip} & 42.8 & 71.6 & 81.1 & 65.2 & 41.4 & 70.6 & 80.5 & 64.2 & 1 & 4 \\
% BridgeFormer\cite{bridgeformer} & 44.9 & 71.9 & 80.3 & 65.7 & - & - & - & - & 1 & 4 \\
% CLIP2Video\cite{clip2video} & 44.9 & 72.2 & 81.3 & 66.1 & 44.4 & 72.3 & 82.2 & 66.3 & 2 & 8 \\
% LAFF\cite{laff} & 45.8 & 71.5 & 82.0 & 66.4 & - & - & - & - & 4 & 16 \\
% TS2-Net\cite{ts2net} & 46.7 & 72.6 & 81.2 & 66.8 & 43.6 & 71.1 & 82.7 & 65.8 & 12 & 26 \\
% X-CLIP\cite{xclip} & 45.3 & 73.7 & 81.9 & 67.0 & 44.9 & 73.4 & 81.9 & 66.7 & 384 & 88 \\
% X-Pool\cite{xpool} & 46.9 & 72.8 & 82.2 & 67.3 & 44.4 & 73.3 & 84.0 & 67.2 & 512 & 26 \\ \hline
% \multicolumn{11}{l}{\textit{X-CLIP as teacher, CLIP4Clip as student}} \\
% TeachCLIP-Coarse & $44.2_{\uparrow1.4}$ & $71.7_{\uparrow0.1}$ & $80.6_{\downarrow0.5}$ & $65.5_{\uparrow0.3}$ & $42.4_{\uparrow1.0}$ & $70.3_{\downarrow0.3}$ & $80.6_{\downarrow0.1}$ & $64.4_{\uparrow0.2}$ & 1 & 4 \\
% TeachCLIP-Fine & $45.2_{\uparrow2.4}$ & $72.3_{\uparrow0.7}$ & $82.3_{\uparrow1.2}$ & $66.6_{\uparrow1.4}$ & $43.6_{\uparrow2.2}$ & $71.3_{\uparrow0.7}$ & $81.6_{\uparrow1.1}$ & $65.5_{\uparrow1.3}$ & 1 & 4 \\ \hline
% \multicolumn{11}{l}{\textit{TS2-Net as teacher, CLIP4Clip as student}} \\
% TeachCLIP-Coarse & $44.0_{\uparrow1.2}$ & $71.3_{\downarrow0.3}$ & $81.1_{\uparrow0.0}$ & $65.5_{\uparrow0.3}$ & $41.2_{\downarrow0.2}$ & $69.5_{\downarrow1.1}$ & $80.5_{\uparrow0.0}$ & $63.7_{\downarrow0.5}$ & 1 & 4 \\
% TeachCLIP-Fine & $45.6_{\uparrow2.8}$ & $72.1_{\uparrow0.5}$ & $81.7_{\uparrow0.6}$ & $66.5_{\uparrow1.3}$ & $43.0_{\uparrow1.6}$ & $71.4_{\uparrow0.8}$ & $81.4_{\uparrow0.9}$ & $65.3_{\uparrow1.1}$ & 1 & 4 \\ \hline
% \end{tabular}
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[ht!]
\caption{\textbf{T2VR performance on MSRVTT-1k}. Baseline models marked with * are our replication using their author-provided source code. Baselines sorted in ascending order by SumR, \ie. sum of R1, R5 and R10.}
\label{table:msrvtt-1ka}
%\setlength{\tabcolsep}{2pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.1} % Default value: 1
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
\textbf{Model} &   R1$\uparrow$ & R5$\uparrow$ & R10$\uparrow$ & SumR$\uparrow$ & \makecell[c]{FLOPs\\(k)$\downarrow$} & \makecell[c]{Store\\(KB)$\downarrow$} \\ \hline
\multicolumn{7}{@{}l}{\textit{Feature re-learning w/o CLIP feature}:} \\
W2VV++ \cite{w2vv++} & 18.9 & 45.3 & 57.5 & 121.7 & 4 & 16 \\
DualE \cite{dualencoding} & 21.1 & 48.7 & 60.2 & 130.0 & 4 & 16 \\
CE \cite{ce} & 20.9 & 48.8 & 62.4 & 132.1 &  &  \\
SEA \cite{sea} & 23.8 & 50.3 & 63.8 & 137.9 & 20 & 80 \\
MMT \cite{mmt} & 24.6 & 54.0 & 67.1 & 145.7 &  & \\
TeachText \cite{teachtext} & 29.6 & 61.6 & 74.2 & 165.4 & 1.5 & 6 \\
\multicolumn{7}{@{}l}{\textit{Feature re-learning with CLIP feature}:}\\
SEA \cite{sea} & 37.2 & 67.1 & 78.3 & 182.6 & 20 & 80 \\
W2VV++ \cite{w2vv++} & 39.4 & 68.1 & 78.1 & 185.6 & 4 & 16 \\
MMT \cite{mmt} & 39.5 & 68.3 & 78.3 & 186.1 &  & \\
LAFF \cite{laff} & 45.8 & 71.5 & 82.0 & 199.3 & 8 & 32 \\
\multicolumn{7}{@{}l}{\textit{CLIP-based end-to-end}:}\\
CLIP4Clip* \cite{clip4clip} & 42.8 & 71.6 & 81.1 & 195.5 & \textbf{1} & \textbf{4} \\
CenterCLIP \cite{centerclip} & 44.2 & 71.6 & 82.1 & 197.9 & 3 & 8 \\
TS2-Net* \cite{ts2net} & \textbf{46.7} & 72.6 & 81.2 & 200.5 & 12 & 26 \\ 
X-CLIP* \cite{xclip} & 45.3 & \textbf{73.7} & 81.8 & 200.8 & 384 & 88 \\
X-Pool* \cite{xpool} & 46.0 & 72.8 & \textbf{82.7} & \textbf{201.5} & 512 & 26 \\
[3pt] %\hline
\emph{This paper}: \\  %\hline
%\multicolumn{7}{l}{\textit{X-CLIP as teacher}} \\
%\multicolumn{7}{l}{\textit{TS2-Net as teacher}} \\
TeachCLIP(TS2-Net) & 45.6 & 72.1 & 81.7 & 199.4 & \textbf{1} & \textbf{4} \\ 
TeachCLIP(X-CLIP) & 45.2 & 72.3 & 82.3 & 199.8 & \textbf{1} & \textbf{4} \\
TeachCLIP(X-Pool) & 44.7  & 73.0  & 82.1 & 199.8 & \textbf{1} & \textbf{4} \\ %\hline
\bottomrule
\end{tabular}
}
\end{table}


% 原始的结果
% CLIP4Clip \cite{clip4clip} & 44.5 & 71.4 & 81.6 & 197.5 & 1 & 4 \\
% X-CLIP \cite{xclip} & 46.1 & 73.0 & 83.1 & 202.2 & 384 & 88 \\
%TS2-Net \cite{ts2net} & 47.0 & 74.5 & 83.8 & 205.3 & 12 & 26 \\

% X-Pool \cite{xpool} & \textbf{46.9} & 72.8 & 82.2 & \textbf{201.9} & 512 & 26 \\

% CLIP2Video \cite{clip2video} & 45.6 & 72.6 & 81.7 & 199.9 & 2 & 8 \\
% BridgeFormer \cite{bridgeformer} & 44.9 & 71.9 & 80.3 & 197.1 & 1 & 4 \\

==> tables/otherdataset.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{table*}[ht!]
\centering
\caption{\textbf{T2VR performance on MSRVTT-3k, VATEX, MSVD and ActivityNet.}}
\label{table:others}
% \setlength{\tabcolsep}{3pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.1} % Default value: 1
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lccrrrrrrrrrrrrrrrrrrrr@{}}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{FLOPs} & \multirow{2}{*}{Store} & \multicolumn{4}{c}{MSRVTT-1k} &\multicolumn{4}{c}{MSRVTT-3k} & \multicolumn{4}{c}{VATEX} & \multicolumn{4}{c}{MSVD} & \multicolumn{4}{c}{ActivityNet} \\ 
\cmidrule(r){4-7} \cmidrule(r){8-11} \cmidrule(r){12-15} \cmidrule(r){16-19} \cmidrule(r){20-23}
 & & & R1 & R5 & R10 & SumR & R1 & R5 & R10 & SumR & R1 & R5 & R10 & SumR & R1 & R5 & R10 & SumR & R1 & R5 & R10 & SumR \\ \hline
\multicolumn{17}{@{}l}{\textit{Feature re-learning w/o CLIP feature}:}\\
W2VV++ \cite{w2vv++} & 4 & 16 & 18.9 & 45.3 & 57.5 & 121.7 & 11.1 & 29.6 & 40.5 & 81.2 & - & - & - & - & 22.4 & 51.6 & 64.8 & 138.8 & - & - & - & - \\
 DualE \cite{dualencoding} & 4 & 16 & 21.1 & 48.7 & 60.2 & 130.0 & 11.6 & 30.3 & 41.3 & 83.2 & 36.8 & 73.6 & 83.7 & 194.1 & - & - & - & - & - & - & - & - \\
 CE \cite{ce} & & & 20.9 & 48.8 & 62.4 & 132.1 & 10.0 & 29.0 & 41.2 & 80.2 & - & - & - & - & 19.8 & 49.0 & 63.8 & 132.6 & 17.7 & 46.6 & - & - \\
 SEA \cite{sea} &  20 & 80 & 23.8 & 50.3 & 63.8 & 137.9 & 13.1 & 33.4 & 45.0 & 91.5 & - & - & - & - & 24.6 & 55.0 & 67.9 & 147.5 & - & - & - & - \\
 MMT \cite{mmt} & & & 24.6 & 54.0 & 67.1 & 145.7 & - & - & - & - & - & - & - & - & - & - & - & - & 22.7 & 54.2 & - & - \\
TeachText \cite{teachtext} & 1.5 & 6 & 29.6 & 61.6 & 74.2 & 165.4 & 15.0 & 38.5 & 51.7 & 105.2 & 53.2 & 87.4 & 93.3 & 233.9 & 25.4 & 56.9 & 71.3 & 153.6 & 23.5 & 57.2 & - & - \\
\multicolumn{17}{@{}l}{\textit{Feature re-learning with CLIP feature}:}\\
SEA \cite{sea} &  20 & 80 & 37.2 & 67.1 & 78.3 & 182.6 & 19.9 & 44.3 & 56.5 & 120.7 & 52.4 & 90.2 & 95.9 & 238.5 & 34.5 & 68.8 & 80.5 & 183.8 & - & - & - & - \\
W2VV++ \cite{w2vv++} & 4 & 16 & 39.4 & 68.1 & 78.1 & 185.6 & 23.0 & 49.0 & 60.7 & 132.7 & 55.8 & 91.2 & 96.0 & 243.0 & 37.8 & 71.0 & 81.6 & 190.4 & - & - & - & - \\
MMT \cite{mmt} & & & 39.5 & 68.3 & 78.3 & 186.1 & 24.9 & 50.5 & 62.0 & 137.4 & 54.4 & 89.2 & 95.0 & 238.6 & 40.6 & 72.0 & 81.7 & 194.3 & - & - & - & - \\
LAFF \cite{laff} & 8 & 32 & 45.8 & 71.5 & 82.0 & 199.3 & 29.1 & 54.9 & 65.8 & 149.8 & 59.1 & 91.7 & \textbf{96.3} & 247.1 & 45.4 & 70.6 & 84.6 & 200.6 & - & - & - & - \\
\multicolumn{17}{@{}l}{\textit{CLIP-based end-to-end}:}\\
CenterCLIP\cite{centerclip} & 3 & 8 &  44.2 & 71.6 & 82.1 & 197.9 & - & - & - & - & - & - & - & - & 47.3 & 76.8 & 85.6 & 209.7 & 43.9 & \textbf{74.6} & \textbf{85.8} & \textbf{204.3} \\
CLIP4Clip* \cite{clip4clip} & \textbf{1} & \textbf{4} & 42.8 & 71.6 & 81.1 & 195.5 & 29.4 & 54.9 & 65.8 & 150.1 & 61.6 & 91.1 & 95.8 & 248.5 & 45.6 & 76.1 & 84.9 & 206.6 & 39.7 & 71.0 & 83.4 & 194.1 \\
 TS2-Net* \cite{ts2net} & 12 & 26 & \textbf{46.7} & 72.6 & 81.2 & 200.5 & 29.9 & 56.4 & 67.3 & 153.6 & 61.1 & 91.5 & 96.0 & 248.6 & 44.6 & 75.8 & 84.5 & 204.9 & 37.3 & 69.9 & 83.2 & 190.4 \\
X-CLIP* \cite{xclip} & 384 & 88 & 45.3 & \textbf{73.7} & 81.8 & 200.8 & \textbf{31.2} & \textbf{57.4} & \textbf{68.1} & \textbf{156.7} & 62.2 & 90.9 & 95.4 & 248.5 & 47.2 & 77.0 & \textbf{85.9} & 210.1 & \textbf{44.4} & \textbf{74.6} & 85.1 & 204.1 \\
X-Pool* \cite{xpool} & 512 & 26 & 46.0 & 72.8 & \textbf{82.7} & \textbf{201.5} & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
[3pt]
\emph{This paper}: \\  %\hline
% \multicolumn{17}{l}{\textit{X-CLIP as teacher}} \\
TeachCLIP(TS2-Net) & \textbf{1} & \textbf{4} & 45.6 & 72.1 & 81.7 & 199.4  & 30.6 & 56.3 & 66.5 & 153.4 & 62.7 & 91.8 & 96.2 & 250.7 & 47.0 & 77.2 & 85.6 & 209.8 & 41.5 & 72.5 & 84.4 & 198.4  \\ %\hline
% \multicolumn{17}{l}{\textit{TS2-Net as teacher}} \\ 
TeachCLIP(X-CLIP) & \textbf{1} & \textbf{4} & 45.2 & 72.3 & 82.3 & 199.8 & 30.4 & 56.3 & 66.7 & 153.4 & \textbf{63.6} & \textbf{91.9} & 96.1 & \textbf{251.6} & \textbf{47.4} & \textbf{77.3} & 85.5 & \textbf{210.2} & 42.2 & 72.7 & 85.4 & 200.1  \\ 
TeachCLIP(X-Pool) & \textbf{1} & \textbf{4} & 44.7  & 73.0  & 82.1 & 199.8 & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ 
\bottomrule
\end{tabular}
}
\end{table*}


%原始结果
% CLIP4Clip \cite{clip4clip} & - & - & - & - & - & - & - & - & 45.2 & 75.5 & 84.3 & 205.0 & 40.5 & 72.4 & - & - \\
% X-CLIP \cite{xclip} & - & - & - & - & - & - & - & - & 47.1 & 77.8 & - & - & 44.3 & 74.1 & - & - \\
%TS2-Net \cite{ts2net} & - & - & - & - & 59.1 & 90.0 & 95.2 & 244.3 & - & - & - & - & 41.0 & 73.6 & 84.5 & 199.1 \\

% X-Pool \cite{xpool} & - & - & - & - & - & - & - & - & 47.2 & 77.4 & 86.0 & 210.6 & - & - & - & - \\

% CLIP2Video \cite{clip2video} & - & - & - & - & 57.3 & 90.0 & 95.5 & 242.8 & 47.0 & 76.8 & \textbf{85.9} & 209.7 & - & - & - & - \\



==> tables/v2t_all_dataset.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!h]
\centering
\caption{\textbf{Video-to-text retrieval performance on multiple datasets}. TeachCLIP uses X-CLIP as the teacher.
% Note that we replicate existing methods with their author-provided source code where applicable, so the numbers might differ (slightly) from their original papers.
%MSRVTT-1k, MSRVTT-3k, VATEX, MSVD and ActivityNet.} Baseline models marked with * are our replication using their author-provided source code.
}
\label{table:v2t_alldatasets}
% \setlength{\tabcolsep}{3pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.1} % Default value: 1
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lrrrrrrrrrrrrrrr@{}}
\toprule
\multirow{2}{*}{\textbf{model}} & \multicolumn{3}{c}{\textbf{MSRVTT-1k}} & \multicolumn{3}{c}{\textbf{MSRVTT-3k}} & \multicolumn{3}{c}{\textbf{MSVD}} & \multicolumn{3}{c}{\textbf{VATEX}} & \multicolumn{3}{c}{\textbf{ActNetCap}} \\
\cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){8-10} \cmidrule(r){11-13} \cmidrule(r){14-16}
 & R1 & R5 & SumR & R1 & R5 & SumR & R1 & R5 & SumR & R1 & R5 & SumR & R1 & R5 & SumR \\ \hline

CenterCLIP \cite{centerclip} & 42.8 & 71.7 & 196.7 & - & - & - & 57.9 & 83.6 & 232.0 & - & - & - & 44.5 & 75.7 & 206.4 \\
TS2-Net \cite{ts2net} & 43.6 & 71.1 & 197.4 & 53.0 & 82.5 & 225.3 & 62.5 & 85.8 & 240.9 & 78.7 & 97.8 & 275.8 & 41.3 & 72.1 & 198.5 \\
X-Pool \cite{xpool} & 45.1 & 73.7 & 202.6 & - & - & - & - & - & - & - & - & - & - & - & - \\ [3pt]

X-CLIP \cite{xclip} & 44.9 & 73.4 & 200.2 & 56.1 & 84.3 & 232.7 & 64.3 & 87.5 & 244.9 & 77.3 & 97.4 & 273.8 & 44.4 & 74.7 & 205.4 \\
CLIP4Clip \cite{clip4clip} & 41.4 & 70.6 & 192.5 & 50.8 & 78.5 & 216.3 & 63.3 & 85.4 & 240.4 &  77.0 & 97.4 & 273.4 & 39.5 & 71.4 & 194.5 \\ 
TeachCLIP & 43.6 & 71.3 & 196.5 & 54.8 & 82.8 & 228.5 & 63.5 & 86.4 & 241.8 & 80.0 & 98.4 & 277.9 & 41.9 & 73.9 & 201.5 \\
\bottomrule
\end{tabular}
}
\end{table*}

%  	 	93.1 	 
% \begin{table*}[]
% \centering
% \caption{\textbf{V2TR Performance of different methods on multiple datasets}.
% % Note that we replicate existing methods with their author-provided source code where applicable, so the numbers might differ (slightly) from their original papers.
% %MSRVTT-1k, MSRVTT-3k, VATEX, MSVD and ActivityNet.} Baseline models marked with * are our replication using their author-provided source code.
% }
% \label{table:v2t_alldatasets}
% % \setlength{\tabcolsep}{3pt} % Default value: 6pt
% \renewcommand{\arraystretch}{1.1} % Default value: 1
% \resizebox{\linewidth}{!}{
% \begin{tabular}{@{}lrrrrrrrrrrrrrrrrrrrrrr@{}}
% \toprule
% \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\makecell[c]{FLOPs\\(k)$\downarrow$}} & \multirow{2}{*}{\makecell[c]{Store\\(KB)$\downarrow$}} & \multicolumn{3}{c}{\textbf{MSRVTT-1k}} &\multicolumn{3}{c}{\textbf{MSRVTT-3k}} & \multicolumn{3}{c}{\textbf{MSVD}} & \multicolumn{3}{c}{\textbf{VATEX}} & \multicolumn{3}{c}{\textbf{ActNetCap}} \\ 
% \cmidrule(r){4-6} \cmidrule(r){7-9} \cmidrule(r){10-12} \cmidrule(r){13-15} \cmidrule(r){16-18}
% & & & R1 & R5 & SumR & R1 & R5 & SumR & R1 & R5 & SumR & R1 & R5 & SumR & R1 & R5 & SumR \\ \hline
% \multicolumn{16}{@{}l}{\textit{Feature re-learning w/o CLIP feature}:}\\
% W2VV++, MM19 \cite{w2vv++} & 2.0 & 8 & 16.9 & 42.7 & 114.2 & 17.5 & 40.2 & 110.2 & - & - & - & 41.8 & 75.1 & 201.2 & - & - & - \\
% DualE, PAMI21 \cite{dualencoding} & 2.0 & 8 & 21.7 & 49.4 & 132.7 & 22.5 & 47.1 & 128.5 & - & - & - & 46.8 & 75.7 & 207.6 & - & - & - \\
% CE, BMVC19 \cite{ce} & 6.1 & 27 & 20.6 & 50.3 & 134.9 & 15.6 & 40.9 & 111.7 & - & - & - & - & - & - & 17.7 & 46.6 & - \\
% SEA, TMM21 \cite{sea} & 10.2 & 40 & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
% MMT, ECCV20 \cite{mmt} & 3.6 & 14 & 24.4 & 56.0 & 148.2 & - & - & - & - & - & - & - & - & - & 22.9 & 54.8 & - \\
% TeachText, ICCV21 \cite{teachtext} & 0.8 & 3 & 32.1 & 62.7 & 169.8 & 25.3 & 55.6 & 149.5 & 27.1 & 55.3 & 149.5 & 64.7 & 91.5 & 252.4 & 23.0 & 56.1 & - \\ [3pt]
% \multicolumn{16}{@{}l}{\textit{Feature re-learning with CLIP feature}:}\\
% SEA & 10.2 & 40 & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
% W2VV++ & 2.0 & 8 & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
% MMT & 3.6 & 14 & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
% LAFF, ECCV22 \cite{laff} & 4.1 & 16 & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\ [3pt]
% \multicolumn{16}{@{}l}{\textit{CLIP-based end-to-end}:}\\
% CenterCLIP, SIGIR22 \cite{centerclip} & 1.5$\sim$7.7 & 6$\sim$30 & 42.8 & 71.7 & 196.7 & - & - & - & 57.9 & 83.6 & 232.0 & - & - & - & 44.5 & 75.7 & 206.4 \\
% CLIP4Clip, Neurocom22 \cite{clip4clip} & 0.5 & 2 & 41.4 & 70.6 & 192.5 & 50.8 & 78.5 & 216.3 & 63.3 & 85.4 & 240.4 &  77.0 & 97.4 & 273.4 & 39.5 & 71.4 & 194.5 \\
% TS2-Net, ECCV22 \cite{ts2net} & 6.1$\sim$32.8 & 24$\sim$128 & 43.6 & 71.1 & 197.4 & 53.0 & 82.5 & 225.3 & 62.5 & 85.8 & 240.9 & 78.7 & 97.8 & 275.8 & 41.3 & 72.1 & 198.5 \\
% X-CLIP, MM22 \cite{xclip} & 220.9$\sim$2175.9 & 26$\sim$130 & 44.9 & 73.4 & 200.2 & 56.1 & 84.3 & 232.7 & xx & xx & xx & 77.3 & 97.4 & 273.8 & 44.4 & 74.7 & 205.4 \\
% X-Pool, CVPR22 \cite{xpool} & 275.0 & 24 & 45.1 & 73.7 & 202.6 & - & - & - & - & - & - & - & - & - & - & - & - \\ [3pt]
% TeachCLIP(X-CLIP) & 0.5 & 2 & 43.6 & 71.3 & 196.5 & 54.8 & 82.8 & 228.5 & 63.5 & 86.4 & 241.8 & 80.0 & 98.4 & 277.9 & 41.9 & 73.9 & 201.5 \\
% \bottomrule
% \end{tabular}
% }
% \end{table*}
